Mind Mappings: Enabling Efficient Algorithm-Accelerator Mapping Space Search

Modern day computing increasingly relies on specialization to satiate growing performance and efficiency requirements. A core challenge in designing such specialized hardware architectures is how to perform mapping space search, i.e., search for an optimal mapping from algorithm to hardware. Prior work shows that choosing an inefficient mapping can lead to multiplicative-factor efficiency overheads. Additionally, the search space is not only large but also non-convex and non-smooth, precluding advanced search techniques. As a result, previous works are forced to implement mapping space search using expert choices or sub-optimal search heuristics. This work proposes Mind Mappings, a novel gradient-based search method for algorithm-accelerator mapping space search. The key idea is to derive a smooth, differentiable approximation to the otherwise non-smooth, non-convex search space. With a smooth, differentiable approximation, we can leverage efficient gradient-based search algorithms to find high-quality mappings. We extensively compare Mind Mappings to black-box optimization schemes used in prior work. When tasked to find mappings for two important workloads (CNN and MTTKRP), the proposed search finds mappings that achieve an average $1.40\times$, $1.76\times$, and $1.29\times$ (when run for a fixed number of steps) and $3.16\times$, $4.19\times$, and $2.90\times$ (when run for a fixed amount of time) better energy-delay product (EDP) relative to Simulated Annealing, Genetic Algorithms and Reinforcement Learning, respectively. Meanwhile, Mind Mappings returns mappings with only $5.32\times$ higher EDP than a possibly unachievable theoretical lower-bound, indicating proximity to the global optima.

==> ASPLOS CR/problem.tex <==
\section{Problem Statement}
During the design process of a hardware accelerator, the architects typically have two decisions to make. 

\paragraph{Architecture} First, to choose architectural parameters to suit the budget and deployment requirements. These can include the number of processing elements, on-chip buffer sizes, network-on-chip type, bandwidth to off-chip memory to name a few. 
Let $A$ represent the architectural space of the exhaustive possibility of these hardware parameters at design time.

\paragraph{Schedule} As the next stage, for those chosen architectural parameters, the algorithm needs to be mapped --- which is the subject of this paper.
These scheduling parameters may be deduced: (1) in design time to be built into the hardware (2) in compile time to be mapped to the hardware, or (3) in run-time to dynamically to mapped to the hardware.
Let $S$ represent the schedule space of all the possible combinations of schedules.

Consider an architecture space $A$, where each architecture $a\in A$ has a schedule space $S$. Let a function $f$ estimate the cost vector $y$ for an input schedule $x\in S$, where the definition of \emph{cost} is upto the designer. Now, we can define the optimization problem that the designer needs to solve formally as Equation~\ref{eq:minmize}.
\begin{equation}
\displaystyle{\minimize_{a\in A} \ \minimize_{x\in S} \ f(a,x)}
\label{eq:minmize}
\end{equation}

The outer minimization problem includes several decisions that are tied to business, which is outside the purview of mathematics. Hence, we restrict our optimization search to finding the best schedule $x_{min}$ that achieves the target objective $y$ for a given architecture $a$, as depicted in Equation~\ref{eq:schedule}.

\subsection{Why is this a hard problem? }
The algorithm mapping to a specialized hardware has been a subject of extensive work in the recent time. Often referred to as the `dataflow', it dictates as to how the data is accessed, managed on-chip, delivered to the compute units, and how the compute is performed and written back.
Every variable that 
This mapping problem is a combinatorial optimization that is np-complete~\cite{npcomplete}, i.e., the solution can be verified in polynomial time. 
\begin{equation}
x_{min} = \argmin_{x\in S} f(a, x)
\label{eq:schedule}
\end{equation}


However, approaches to choose the mapping has either been based on expert designer choices or based on exhaustive searches. While exhaustive search is simply infeasible when all the parameters are enumerated, the designer choice may not be very optimal.

==> background.tex <==
\section{Related Work}
\label{sec:blackbox}

%%%%%%%%%%%%%%%%%%% Detailed Table %%%%%%%%%%%%%%%%%%% 
\begin{table*}[!t]
\centering
\caption{Related works in Mapping Space Search. Mind Mappings differentiates from other works by enabling a first-order optimization using Gradient Descent with a differentiable surrogate.
% \chris{somehow bring out WB vs BB.  cost function and search heuristic isn't telling me why you are better}
% \chris{why isn't the MLP from Adams et al. also differentiable?}\kartik{It is, but not used for the same thing as us}
}
\begin{tabular}{c|c|c|c} 
 \hline
 \textbf{Work} & \textbf{Problem Domain} & \textbf{Cost Function} & \textbf{Search Heuristic}  \\ [0.5ex] 
 \hline\hline
 FlexTensor~\cite{flextensor} & Tensor Compilation & Actual Hardware & Reinforcement Learning \\
 Tiramisu~\cite{tiramisu} & DNN Compilation & Actual hardware & Beam Search \\
 Gamma~\cite{gamma} & DNN Mapping Space Search & Analytical & Genetic Algorithm \\
 TensorComprehensions~\cite{tensorComprehensions} & DNN Compilation & Actual hardware & Genetic Algorithms \\
   dMazeRunner~\cite{dmazerunner} & DNN Compilation & Analytical & Pruned Search \\
 Timeloop~\cite{timeloop} & Affine loop nests & Analytical & Pruned Search  \\
 TVM~\cite{tvm} & DNN Compilation & Gradient Boosted Trees & Simualted Annealing  \\
 RELEASE~\cite{release} & DNN Compilation & Gradient Boosted Trees\ & Reinforcement Learning \\ 
 Adams et. al~\cite{beamsearch_halide} & Halide~\cite{halide} Compilation & Multi-Layer Perceptrons & Beam Search \\

%  STOKE~\cite{stoke} & General? & TODO & MCMC Sampling? TODO \\
 \textbf{Mind Mappings (ours)} & \textbf{Domain Agnostic} & \textbf{Multi-Layer Perceptrons} & \textbf{Gradient-based  Search} \\ [1ex] 
 \hline
\end{tabular}
\label{table:related_work}
\end{table*}
%%%%%%%%%%%%%%%%%%% \ Detailed Table %%%%%%%%%%%%%%%%%%% 

%Algorithm-accelerator mapping space search described in Section~\ref{subsec:mapspace_search} is a difficult combinatorial search problem, where the accelerator cost model is a black box, i.e., one not obtain information such as gradients, Hessians, etc., other than the ability to evaluate the function itself.
%Additionally, the cost model is non-convex~(Section~\ref{subsec:mapspace_example}), further complicating the search.
%Due to this, prior works employ black-box optimization techniques such as Simulated Annealing, Genetic Algorithms, Reinforcement Learning, etc., to solve the mapping space search problem.
%Mind Mappings differentiates from prior works by enabling first-order optimization using gradients, by approximating the search space with a differentiable surrogate.
%Table~\ref{table:related_work} lists prior works in this area and their approach to solve the mapping space search problem.

%\chris{Again, above several sentences are a bit disconnected.  First sentence: which black-box search problem?}\kartik{Changed to mapping space search problems}
% While an extensive literature exists for classic black-box optimization problems, mapping space search has its own unique characteristics, challenges, and opportunities.

We now describe prior work studying mapping space search as well as related search techniques applied to other problems.
We summarize the former in Table~\ref{table:related_work}.

%, we throw light on prior work on mapping space search problems as well related works in other areas whose ideas can be incorporated to mapping space search.

%\chris{The above writing could be improved.
%The first two sentences are both topic sentences.  
%The last sentence describes the first sub-section but not the second sub-section.
%This is also the first time where ``black box'' comes up, and should probably be re-defined.}

% \chris{Nota bene: When ``black-box'' is used as a compound adj, add a hyphen.  If it is used as a noun (as above), it should not have a hyphen}

% Search methods have two key components.
% First, a \emph{cost model} that can accurately calculate the cost of a solution.
% Second, a \emph{search heuristic} that can propose high quality solutions that minimize the overall cost.

% \subsubsection{Cost Models: Learned vs Actual}
% \label{subsec:cost_models}
% Cost model is the implementation of $f(x)$ described in Equation~\ref{eq:schedule} and is the black-box we are trying to optimize.
% A straight-forward way to generate the cost is by evaluating the mapping on an actual hardware or a representative model of the same, which we term as \emph{actual} cost model.
% While being accurate in predicting the cost, this approach is the slowest to execute.
% This hampers the search methods by limiting the number of samples.
% Instead, the cost models can be approximated by learning a mapping function $f^*(x)$, which we refer to as a \emph{learned} cost model.
% They can be trained based on the real cost model to best approximate the cost $f(x)$.

% \subsubsection{Search Heuristics: Guided vs Unguided}
% \label{subsec:search_heuristics}

% Given the large search space size, an exhaustive search is not feasible.
% Therefore, a heuristic based search is necessary.
% Such heuristics can be learnt during the run-time based on the behavior of the cost function, which we term as an \emph{unguided} search.
% Or, the search can utilize some pre-learned heuristics to steer the search in the right direction, which we call as a \emph{guided} search.
% While the guided search has the potential to perform better than its counterpart, a key difficulty in enabling a guided search is in the ability to develop a generalized heuristic that can apply to any shape of the problem.

% A key insight from this work is that the learned cost model itself can serve as a generalized heuristic to enable a guided search in the search space.
% We enable this by using a differentiable model to learn the actual cost model, then by generating gradients from such a differentiable model to generate the solutions. We elaborate on our proposed method in Section~\ref{sec:method}.

\subsection{Mapping Space Search}
\label{subsec:surrogate_related}

% \chris{Table 2 says the other works DO NOT do mapping space search.  But this section says they do because the sub-section heading is called mapping space search.}

%%%%%%%%%%%%%%%%%%% Simpler Table %%%%%%%%%%%%%%%%%%% 
% \begin{table*}[t]
% \centering
% \begin{tabular}{c|c|c|c|c} 
%  \hline
%  \textbf{Work} & \textbf{General to any domain} & \textbf{Learned Cost Model} & \textbf{Guided Search } & \textbf{Target Hardware} \\ [0.5ex] 
%  \hline\hline
%  Timeloop~\cite{timeloop} & Constrained & No & No & Acc. \\ 
%  TVM~\cite{tvm} & No & Yes & No & CPU/GPU/Acc. \\ 
%  Adams et al~\cite{beamsearch_halide} & No & Yes & No & CPU \\
%  Tiramisu~\cite{tiramisu} & Constrained & TODO & No & CPU/GPU \\
%  dMazeRunner~\cite{dmazerunner} & No & No & No & Accelerators \\
%  TensorComprehensions~\cite{tensorComprehensions} & No & TODO & No & CPU/GPU \\
%  RELEASE~\cite{release} & No & Yes & No & CPU/GPU/Acc. \\ 
%  STOKE~\cite{stoke} & General? & TODO & No & CPU \\
%  Mind Mappings (ours) & Yes & Yes & Yes & Accelerators \\ [1ex] 
%  \hline
% \end{tabular}
% \caption{Related works in mapping space search. \kartik{Angshu/Po-An, shome works here can potentially be general, but the paper does not explore the same, classify them as "potential"?}}
% \label{table:related_work}
% \end{table*}
%%%%%%%%%%%%%%%%%%% \ Simpler Table %%%%%%%%%%%%%%%%%%% 

% While targeting different problem domain, 
To overcome the challenges in mapping search space, prior works use two main approaches:
~(i) reduce the time to evaluate the cost function, and
~(ii) avoid exhaustive search by adopting better heuristics.

\subsubsection{Faster Cost Estimation.}
\label{sec:related:fast_estimation}

For unguided mapping space search techniques that rely on exhaustive search or black-box methods, evaluating more mappings is the key to find higher-quality mappings.
However, a key challenge is that the cost to evaluate a mapping using the actual hardware or a representative simulator is non-trivial.
To get around this, prior works use several techniques, described below.

%\chris{For below sub-sub-sections, the first sentence should give the main idea}
%\chris{Above sentence isn't crisp.  It isn't clear until the end of the sentence why running on real HW is bad, hence the middle is confusing.}
%\kartik{Fixed both}

dMazeRunner~\cite{dmazerunner}, Timeloop~\cite{timeloop}, GAMMA~\cite{gamma}
use analytical models built by domain experts that are faster to evaluate than the actual hardware, and are sufficiently representative and flexible to support different mappings.
However, building such analytical models is difficult and requires strong domain expertise.
Some other works instead do away with domain expertise requirements by
leveraging machine learning to build an approximate cost function.
%\chris{Above not sentence grammatical}\kartik{Check.}
For example, AutoTVM~\cite{tvm} and RELEASE\cite{release} use gradient-boosted trees~\cite{xgboost}.
On the other hand, Adams et al.~\cite{beamsearch_halide} use Multi-layer Perceptrons (MLPs). % to speed up the performance evaluation (cost function). %
%\chris{should be "et al." not "et. al".  Fix everywhere}
% \chris{last part of sentence sounds redundant.}
% to build a surrogate model to improve the speed of evaluation for compiling and optimizing Halide~\cite{halide} programs on different target platforms.
We note that while we also use MLPs to build the surrogate,
% to simplify the cost function and evaluate solutions faster.
we utilize the \emph{differentiability} of the surrogate to perform a guided search.
%\chris{rewrite to avoid passive voice}
%\chris{use consistent notation for citations.  sometimes you use et al, sometimes you cite directly.  I suggest using the former and when what you are referring to is clear, replace with a reference, e.g., "unlike that work"}
% we focus on building a \emph{differentiable}, multi-layer perceptrons model,
% which is not only cheap for evaluate mappings, but also \emph{provides guidance} for 
% our search heuristics. 

%\chris{Again, below first sentence should be structured to be parallel with first sentence of previous sub-sub-section.  E.g., ``Orthogonal to cost function performance,...''}

\subsubsection{Mapping Space Search with Heuristics.}

Orthogonal to techniques mentioned in Section~\ref{sec:related:fast_estimation} that speed up the cost evaluation, prior works also develop custom/learnt heuristics to improve the search itself, so as to avoid brute-force search.
dMazeRunner~\cite{dmazerunner}, Marvel~\cite{marvel} and Timeloop~\cite{timeloop} prune the search space to reduce the number of mappings that need to be evaluated using domain expert knowledge.
% \chris{why is prune in emph?}
The key idea is that points in the search space can be eliminated without evaluation, e.g., tile sizes 
that do not fit in the on-chip buffer.
%\chris{Above sentence can be stated better.  ``The main idea is that invalid mappings need not be evaluated, e.g., ... .''}
Again, this solution is difficult to scale 
% \chris{difficult to scale}
since it requires extensive domain expertise to create rules to prune the search space.

%\chris{Suggest adding a paragraph header.  "Other works." or similar}
Several prior works leverage black-box optimization methods to perform the search.
%\chris{"to search over ..." could be removed}
For example, AutoTVM uses parallel simulated annealing~\cite{simanneal}~(SA) to search through the map space. 
OpenTuner~\cite{opentuner} is a program auto-tuner that uses the AUC Bandit Meta technique to combine several methods such as differential evolution.
RELEASE~\cite{release} and FlexTensor~\cite{flextensor} both use Reinforcement Learning (RL) as the cost heuristic to guide the search.
Tiramisu~\cite{tiramisu} and Adams et al~\cite{beamsearch_halide} both employ beam search. % to solve the combinatorial search problem.
Finally, TensorComprehensions~\cite{tensorComprehensions} and GAMMA~\cite{gamma} use Genetic Algorithms~\cite{ga_source}, which are a popular approach used in combinatorial optimization~\cite{ga_usage, ga_app_0,ga_app_1}.

For all of the above: 
by definition of being black box, heuristics can only guide the search based on previously visited samples, and therefore require a large number of samples to perform well.
As demonstrated in Section~\ref{sec:eval}, Mind Mappings outperforms SA, GA, and RL by utilizing powerful gradient-based optimization with the differentiable surrogate.
%\chris{the above paragraph needs a punchline.  also, the treatment of different schemes is inconsistent.  E.g., what is the downside of RL, beam search and the AUC bandit meta technique?}
%\kartik{Addressed all the black-box techniques generally}
% However, SA is a meta-heuristic search 
% \chris{what is a meta-heuristic?  is it a bad thing?}
% and its statistical guarantees of finding the global minima is only true 
% \chris{only hold when the problem is convex?}
% for a convex optimization problem.
% \chris{previous sentence: I don't see how we are any better}

% RL heavily relies on the effectiveness of the agent in balancing exploration and exploitation of the search space. 
% \poan{so why does it not work?}

% % However, they use XXX to minimize the run-time of the cost evaluation. \angshu{use what?}\poan{yeah, what?}
%  However, GA's underlying assumption that cross-over of two strong individuals in a population should result in stronger children is not true in mapping space search, thus reducing its effectiveness. 
% % \angshu{I changed the wording of the previous sentence because it had a double-negative and was parsing incorrectly. Please review and see if "should" is too strong of an assertion here.}
% For example, a good tiling for a loop order may not do well with a good loop order for another tiling.

\subsection{Related Works in other Areas}
Beyond mapping space search, the combinatorial search represented in Equation~\ref{eq:schedule} is widely found in other areas such as neural architecture search~\cite{NAS_rl}, device placement~\cite{clite}, etc., and insights from related works in these areas can apply to the mapping space search problem.
% \chris{apply to the map space search problem ... or are helping in solving ...}

\textbf{Surrogate Modeling.} Using surrogates for solving black-box optimization problems has been well explored~\cite{surrogate_modeling}.
To predict the performance of a program on a CPU, Ithermal~\cite{ithemal} and Difftune~\cite{difftune} use Recurrent Neural Networks, {\"I}pek et al.~\cite{surrogate_0} use Artificial Neural Nets, and Lee et al.~\cite{surrogate_1} use regression modeling.
% \chris{make citation style consistent.  see above comments}
Deep generative models are proposed as a surrogate in ~\cite{surrogate_2}, which are differentiable approximations.
Function approximation or surrogate modeling has been at the core of modern Reinforcement Learning methods to approximate the large state-space present in real-life problems.
Similarly, Mind Mappings uses a differentiable surrogate, while carefully tuning the supervised training methods to adapt to the mapping space search problem.

%\chris{above para: what is the punchline?  Do all of those works (esp DiffTune) really just use the surrogate in a BB fashion?}

\textbf{Search Heuristics.}
Black-box approaches such as Simulated Annealing, Genetic Algorithms~\cite{ga_usage, ga_app_0,ga_app_1}, Bayesian Optimization~\cite{bayesian_dnn_0, clite, brandon}, etc., have been widely used in different applications.
Recent advances in Reinforcement Learning~(RL) have influenced several works~\cite{NAS_rl, haq} to adopt the same, with promising results.
Several works have explored gradient-based methods~\cite{fbnet, darts,surrogate_2, difftune}, in spite of the cost function being non-differentiable. For example, FBNet~\cite{fbnet} uses Gumbel-Softmax~\cite{gumbel} to make the discrete choices in their problem differentiable, thereby obtaining gradients.

While gradient-based optimization applied to combinatorial optimization problems with black-box cost functions is not new~\cite{fbnet, darts,surrogate_2, difftune, gradient_technique_0, gradient_technique_1, gradient_technique_2, gradient_technique_3, gradient_technique_4}, adapting this to the mapping space search problem---the focus of this paper---is new and faces non-trivial challenges (Section~\ref{sec:method}).
%We describe the Mind Mappings approach to apply gradient-based approach for mapping space search in Section~\ref{sec:method}.
%\chris{Again, what is the punchline?}

% Neural architecture search~(NAS) tries find a DNN architecture that achieves the best accuracy for a given task, thus forming a similar search problem as algorithm-accelerator mapping space search. Approaches vary from reinforcement learning~\cite{NAS_rl}, Bayesian optimization~\cite{bayesian_dnn_0}, and gradients~\cite{fbnet}. 

% All the prior works utilize black-box optimization methods to perform the search, whose cost is proportional to the search space itself, making it difficult to find high quality mappings in short time.
% % As shown in Section~\ref{sec:intro}, all these black-box optimization methods still have a worst-case search cost proportional to the total size of the search space, and as we will show later in the paper~(Section~\ref{sec:eval}),
% % they cannot reach to a high-quality result in a reasonable time.
% On the contrary, our search heuristic leverages the differentiable characteristic of the surrogate,
% and perform an efficient guided search in the search space using gradients.
% This insight makes our approach search much faster and reach better solutions.


% Genetic Algorithms~(GA)~\cite{ga_source} is a widely adopted~\cite{ga_usage, ga_app_0,ga_app_1} approach for black-box optimization problems and ~\cite{tensorComprehensions} uses the same to obtain efficient mappings.
% GA builds an initial population of solutions and improvises over them by cross-overs and mutations.
% GA's underlying assumption of cross-over of two strong individuals in a population may not result in a stronger children is not true in mapping space search, thus reducing its effectiveness.
% For example, a good tiling for a loop order may not do well with a good loop order for another tiling.

% \subsection{Other Areas dealing with a Large Search Space}
% \poan{honestly, I don't know why we need to mention them. Aren't they the "unrelated" related work that should come at the end of the paper?}
% Neural architecture search~(NAS) tries find a DNN architecture that achieves the best accuracy for a given task, thus forming a similar search problem as algorithm-accelerator mapping space search. 
% Approaches vary from reinforcement learning~\cite{NAS_rl}, Bayesian optimization~\cite{bayesian_dnn_0}, and gradients~\cite{fbnet}. FBNet~\cite{fbnet} defines a macro-architecture and uses Gumbel-Softmax~\cite{gumbel} to make the discrete choice of different block in the macro-architecture differentiable; hence obtaining the gradients to minimize the loss.

% Several recent efforts also utilize machine learning for better heuristics~\cite{tiramisu, ml_comp_0, ml_comp_1, rstream} for code optimization.
% Ithermal~\cite{ithemal} uses DNNs to predict the throughput of a program on general purpose processors.
% Halide~\cite{halide} is a domain-specific language for image processing that opens up opportunities to perform better scheduling and ~\cite{halide_search} uses stochastic searches over Halide's schedule space.

% % %\chris{Most general comment: This section is too generic.  Change the terminology to apply to the map space search problem specifically.}
% Black-box optimization is a core primitive with applications in many areas ranging from mechanical engineering, automotive design, machine learning, etc.---where the systems are difficult to model with a mathematical function~\cite{blackbox}.
% The goal in black-box optimization is to find the $\argmin_{x\in X} f(x)$ of a function $f(x)$, where we do not have any other information about the function other than the ability to evaluate $f(x)$.
% As discussed in Section~\ref{sec:background:challenges}, with a non-smooth, non-convex, non-differentiable cost function, accelerator-algorithm mapping space search is a black-box optimization problem.

% We evaluate traditional black-box optimization methods relative to our proposed approach in Section~\ref{sec:eval}, and thus give a brief overview of them here.
% \todo{Consider making this section as related work, and point out what current works do.} 
% %Due to its wide adoption in areas such as mechanical engineering, automotive design, machine learning, etc., where the systems are difficult to model with a mathematical function.
% %Unsurprisingly, a lot of attention has been given to this important optimization problem, and in this section we give a brief overview of a few effective methods for the same.

% \subsection{Random Walk}
% \label{subsec:rand_walk}
% A straightforward way to improve search performance over an exhaustive search is to perform a random walk in the search space.
% The walk is performed for a fixed number of iterations---where each iteration mutates the input $x$---and the best point during the walk is returned as the solution.
% As the number of iterations increased, the solution quality increases.

% \subsection{Hill climbing}
% \label{subsec:hill_climb}
% Instead of random moves performed in a random walk, hill climbing~(HC) chooses moves which improve the cost.
% A neighboring point is chosen and a move is made only if it improves the existing solution.
% If the function is convex, then HC converges in a global minimum, else it has the danger of getting stuck in local minima.
% Several flavors of HC are deployed in practice such as stochastic HC, random-restart HC, etc.

% \subsection{Simulated Annealing}
% \label{subsec:sim_anneal}

% Simulated Annealing~(SA)~\cite{simanneal} combines both random walk and HC to improve the search efficiency.
% In SA, the next move is chosen randomly as in random walk, but a move is made with probability 1 if it improves the solution, or with a probability $p<1$ if it degrades the solution.
% The value of $p$ is exponentially decayed based on how much worse the next move is with respect to the current solution, and is annealed over the search iterations.
% An example probability function is $p(x) = 1 - \exp^{\frac{-\Delta Y}{T}}$, where $\Delta Y$ is the difference between the cost of the current solution and the next step and $T$ is a temperature that is annealed over the iterations.

% \subsection{Genetic Algorithms}
% \label{subsec:genetic}

% %\chris{this one is going to need more detail to understand eval.  E.g., how is cross-over done?}
% %\kartik{Each 'individual' (mapping) has $d$ 'genes' (prog attributes), and during crossover d/2 of them are exchanged between two parents to produce an off-spring. Mutation is when one of the d genes is randomly changed. The population is evaluated and then fittest individuals are chosen for mating again. This process continues.}

% Genetic Algorithms~(GA)~\cite{genetic} are a class of search method inspired by the theory of natural selection and model the same to choose the fittest individual that minimizes the cost.
% The algorithm begins by creating a population of individuals (mappings) randomly chosen in the search space.
% During the run, a part of the population is selected based on a policy such as best fitness (cost), or round-robin, or randomly etc.
% The selected part of population then undergoes mutations and cross-overs.
% In our setting:
% (1) mutation randomly changes one of the $d$ attributes in the mapping.
% (2) cross-over exchanges $d/2$ attributes between two parents to form a new mapping (offspring).
% If either of these create an invalid mapping, that mapping is dropped, i.e., because it has low fitness.
% This process is repeated until the goal is reached.

% %Intuitively, at every step, this improves the quality of solutions and operators such as cross-over and mutation balance both the \emph{exploitation} and \emph{exploration}.

% \subsection{Bayesian Optimization}
% \label{subsec:bayes_opt}

% %\chris{same as genetic.  need some text to make this concrete for mapping space search} 
% %\kartik{Create a domain of possible values for each of the d attributes and let BO sample from this and build a posterior. TimeLoop is passed as a cost function to evaluate each point.}
% Based off of the famous Bayes theorem, Bayesian Optimization~(BO) consists of two key features: surrogate modeling and acquisition functions.
% Surrogate modeling takes in a prior distribution for each of the $d$ attributes in a mapping, that has some prior knowledge of the search space, and then repeatedly samples from the search space to update the distribution to a posterior distribution that better approximates the search space.
% A Gaussian process is often deployed to enable an effective modeling of the search space.
% The acquisition function helps to direct the sampling mechanism towards areas of the search about which there is a higher possibility of a better solution.
% Each mapping sampled from the posterior is evaluated via the cost function.


% \chris{need TVM, Halide}
% There has been a large number of works that proposed application specific hardware accelerators for diverse areas of computing.
% Majority of the works do not elaborate on their methodology to obtain an efficient mapping of the algorithm, pointing to the human expert-based mapping choices.

% \subsection{Compiler Optimizations.}
% Early works explored loop-transformations such as loop-interchanges, -blocking, -fusion, etc., for improving performance and studied their validity~\cite{loop_transform}.
% A rich literature targeting the automation of such transformations guided by polyhedral models.
% They have been used both for general purpose code optimization such as Polly~\cite{polly} and for specialized requirements such as vectorization~\cite{polyhedral_vectorize}, CUDA~\cite{polyhedral_GPU}, and TensorFlow~\cite{tensorflow_polyheadral}.
% Several recent efforts also utilize machine learning for better heuristics~\cite{tiramisu, ml_comp_0, ml_comp_1, rstream} for code optimization.
% Ithermal~\cite{ithemal} uses DNNs to predict the throughput of a program on general purpose processors.
% Halide~\cite{halide} is a domain-specific language for image processing that opens up opportunities to perform better scheduling and ~\cite{halide_search} uses stochastic searches over Halide's schedule space.

% \subsection{Hardware Accelerators.}
% Given the importance of finding the right hyperparameters for a specialized hardware, several previous works attempted to improve the efficiency of combinatorial searches in hardware design. 
% \cite{brandon} explores Bayesian optimization to simultaneously tune hyperparameters of a DNN and the hardware accelerator for efficiency.
% Pruning the search space effectively is also an attractive avenue for efficient design space searches~\cite{design_space_search_0}.
% TVM~\cite{tvm} uses a gradient boosted tree~\cite{xgboost} to speed-up the performance evaluation and uses parallel simulated annealing~\cite{simanneal} to search through the map space.
% Tensor Comprehensions~\cite{tensorComprehensions} uses Genetic Algorithms, while RELEASE~\cite{release} uses Reinforcement Learning.
% Morph~\cite{morph} uses a pruned map space to perform an exhaustive search for a flexible hardware accelerator.
% Several flexible accelerator designs such as \cite{dna, flexiflow, maeri} do not elaborate on the search strategy, leaving this as an open problem.

% \subsection{Neural Architecture Search}
% Neural architecture search~(NAS) tries find a DNN architecture that achieves the best accuracy for a given task, thus forming a similar search problem as algorithm-accelerator mapping space search. Approaches vary from reinforcement learning~\cite{NAS_rl}, Bayesian optimization~\cite{bayesian_dnn_0}, and gradients~\cite{fbnet}. FBNet~\cite{fbnet} defines a macro-architecture and uses Gumbel-Softmax~\cite{gumbel} to make the discrete choice of different block in the macro-architecture differentiable; hence obtaining the gradients to minimize the loss.

==> conclusion.tex <==
\section{Conclusion}

This paper proposed Mind Mappings, an efficient method for performing algorithm-accelerator mapping space search.
The key idea is to approximate the non-differentiable accelerator cost function with a differentiable surrogate, and to use that surrogate to perform a powerful Gradient Descent-based search.

While Mind Mappings significantly closes the gap to finding optimal mappings quickly, there is still gap left to close.
In particular, Section~\ref{sec:method} details several areas where the method can be further optimized, ranging from improved sampling methods for training the surrogate to more efficient encodings of accelerator programmable attributes.
Long term and with these refinements, we hope that the methods in this paper advance mapping space search to a level closer to its more mature cousin, compilation for general-purpose devices.

%A crucial open problem in hardware accelerator design is to perform an effective algorithm-accelerator mapping space search, which holds the key to a unlock considerable efficiency gains.
%As the first work to comprehensively address this search problem, we formally defined the search problem and proposed a gradient-based search method that outperforms several traditional methods for black-box optimization applied to this search problem.

%We identify several future avenues to improve the work, ranging from developing a better sampling methods in the map space to exploring improved mapping and cost representations for effective surrogate modeling.

%With the combination of significant recent advances in the area of deep learning and the paradigm shift in the architecture community towards specialized hardware design, we believe the time is ripe to utilize deep learning techniques to build efficient hardware accelerators.
% We hope that this work influences future works in this area.

%\chris{Add ACK section}
%\chris{do a pass on references to make their formatting consistent}


==> evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

We now evaluate Mind Mappings.
We design representative flexible hardware accelerators using Timeloop~\cite{timeloop} and search through their map spaces in the context of two target algorithms, while comparing against several other search methods.

%using Mind Mappings and compare it to traditional approaches described in Section~\ref{sec:blackbox} for different workloads.
%\chris{? this needs to mention target algorithm...}

\subsection{Experimental Setup}

\subsubsection{Algorithms}

We evaluate Mind Mappings by evaluating %applying it to the accelerator-algorithm mapping space search for a hardware accelerator for 
two target algorithms, Convolutional Neural Networks~(CNN) and Matricized tensor times Khatri-Rao product~(MTTKRP).
We evaluate two target algorithms to demonstrate generality, and selected these two in particular given the ongoing effort in the architecture community to build efficient hardware accelerators for CNNs~\cite{eyeriss, DaDianNao, shidiannao, scalpel, scnn, cnvlutin, ucnn} and MTTKRP~\cite{extensor,tensaurus}.
CNN layers feature similar, but higher-dimensional, computations as our 1D-Conv example from Section~\ref{subsec:mapspace_example}.

\textbf{CNN-Layer.} 
CNNs have seen widespread success in modern Deep Learning applications such as image recognition, video analytics etc. 
A CNN layer takes $N$ 2D images of resolution $W \times H$ with $C$ channels and $K$ filters of resolution $R \times S$ and produces an output of size $X \times Y$ with $K$ channels.
Value of $X$ and $Y$ can be calculated 
% \chris{why estimated as opposed to computed?  NB: you use the term estimated a lot when I think computed is what you mean.}
from $W$ and $H$ respectively as $(W-R+1)/stride$ and $(H-S+1)/stride$, respectively.
Mathematically, a CNN Layer 
%\chris{it is either ``a CNN layer'' or ``CNN-layer'' depending on whether you are talking about some CNN layer or this benchmark (by its name) specifically.  Which do you mean?}\kartik{I think I just mean the algorithm. I guess hyphen goes off (removed)}
is given by Equation~\ref{eq:conv2d}.

\begin{align}
&\out[(k, x, y)] = 
    \sum_{c=0}^{C-1} \sum_{r=0}^{R-1} \sum_{s=0}^{S-1} 
        \filt[(k, c, r, s)] * \inp[(c, x+r, y+s)] \label{eq:conv2d} \\
    \nonumber &0 \le k < K, 0 \le x < W-R+1, 0 \le y < H-S+1
\end{align}

\textbf{MTTKRP.} MTTKRP~\cite{mttkrp} is a key kernel in Tensor Algebra that is a bottleneck in applications such as tensor decompositions~\cite{kolda_survey}, alternating least squares~\cite{als}, Jacobian estimation~\cite{mttkrp_use}, etc.
MTTKRP takes a 3D tensor $A$, and matrices $B$ \& $C$ to produce and output matrix by contracting across two dimensions, as described in Equation~\ref{eq:mttkrp}.
% \begin{equation}
%     Z_{ij}= \sum\nolimits_{kl} A_{ikl} B_{kj} C_{lj}
%     \label{eq:mttkrp}
% \end{equation}

\vspace{-3mm}
\begin{align}
&\out[(i,j)] = 
    \sum_{k=0}^{K} \sum_{l=0}^{L}
        A[(i,k,l)] * B[(k,j)] * C[(l,j)] \label{eq:mttkrp} \\
    \nonumber \nonumber \ \ \ &0 \le i < I, 0 \le j < J
\end{align}
 \vspace{-3mm}
 
% We refer the readers to appendix for mathematical expressions for both the workloads.

\begin{table}[h]
\centering
\caption{Target problems for each target algorithm.}
\label{tab:problem_shapes}
\begin{tabular}{c|c|c|c|c|c}
    \hline
    \hline
    \textbf{CNN/MTTKRP} & \textbf{N/I} & \textbf{K/J} & \textbf{H,W/K} & \textbf{R,S} & \textbf{C/L} \\
    \hline
    \hline
    ResNet Conv\_3 & 16 & 128 & 28 &  3  &128\\ %6
    ResNet Conv\_4 & 16 & 256 & 14 & 3 &256\\ %7
    Inception Conv\_2 & 32 & 192 & 56  & 3 &192\\ %3
    VGG Conv\_2 & 16 & 128 & 112 & 3  &64\\ %1
    AlexNet Conv\_2 & 8 & 256 & 27  & 5  &96\\ %4
    AlexNet Conv\_4 & 8 & 384 & 13  & 3  &384\\ %5
    MTTKRP\_0 & 128 & 1024 & 4096 & - & 2048 \\
    MTTKRP\_1 & 2048 & 4096 & 1024 & - & 128 \\
    \hline
\end{tabular}
\end{table}


Table~\ref{tab:problem_shapes} shows the target problems we evaluated in Phase 2 %our accelerators with 
for each algorithm.
Specifically, we chose layers from popular networks such as ResNet~\cite{Resnet}, VGG~\cite{vgg}, AlexNet~\cite{Alexnet}, and Inception-V3~\cite{inception} and representative matrix shapes (tall and skinny~\cite{tall_skinny}) for MTTKRP.
%\chris{not sure why we say the above is representative for MTTKRP.  You need to cite something.}\kartik{I used tall and skinny(i guess short fat),a dded cite}
% We remark that Mind Mappings is applicable to any problem of the target algorithm, as the surrogate generalizes over the family of problems for the given algorithm.
% The chosen problem shapes represent different extremes and representative hyper-parameters and are meant to push search methods to check corner cases.
% For example, Inception Conv\_2 has huge inputs and fewer filters, where as AlexNet Conv\_4 has small inputs and large number of filters.
% We remark that the proposed approaches are general and apply to any valid problem dimension.

\subsubsection{Hardware Accelerators}

We model the programmable hardware accelerator using Timeloop~\cite{timeloop}, which uses an analytical cost model to provide a high-fidelity cost estimation for hardware accelerators that implement affine loopnests.

The hardware accelerators we evaluate for both algorithms have the same memory hierarchy, namely
a two-level hierarchy with 512~KB of shared buffer and 64~KB of private buffer for each of 256 processing elements~(PEs). 
Buffers are banked and can be flexibly allocated to store any algorithm operand/partial result (tensors in the case of our target algorithms).
Each level of the memory hierarchy is coupled with control and address generation logic to support any loop order and tile size (similar to \cite{morph}).
The Network-on-Chip~(NoC) provides parallelism across the PEs along any combination of problem dimensions.

For each algorithm, we further specialize the datapath and control logic in PEs and the rest of the accelerator.
For CNN-Layer, PEs can consume 2 operands to produce 1 output per cycle, while for MTTKRP, PEs consume 3 operands to produce 1 output per cycle.
We assume the accelerator runs at 1~GHz and that the design objective is to minimize the energy-delay product~(EDP) to evaluate a problem.
%\chris{problem instance?  do you mean problem?  (if what you mean by problem instance is "mapping" - just say that.}\kartik{Fixed.}

\begin{figure*}[ht]
  \includegraphics[width=\textwidth]{ASPLOS CR/main_result/iso-iter_results.png}
\caption{Iso-iteration comparison of various search methods compared to Mind Mappings (MM).}
\label{fig:main_res_iters}
\end{figure*}

\subsubsection{Map Spaces}
\label{sec:eval:map_spaces}

Given the accelerator architecture $a$ and target problem $p$, each mapping $m \in M_{a,p}$~(Section~\ref{sec:method:input_rep}) 
is defined by the following programmable attributes for CNN-Layer/MTTKRP, typical in recent accelerators~\cite{eyeriss, scnn, ucnn, morph, flexiflow, maeri}.
\begin{enumerate}
    \item \textbf{Tiling:} The tile sizes for each dimension~(7/4) for each of the 3 levels in the memory hierarchy~(\emph{DRAM, L2, and L1}). (21/12 attributes for CNN-Layer and MTTKRP, respectively.)
    \item \textbf{Parallelism:} The degree of parallelism for each dimension across the PEs. (7/4 attributes.)
    \item \textbf{Loop Orders:} The ordering for each dimensions for each of the 3 memory hierarchies. (3/3 attributes.)
    \item \textbf{Buffer Allocation:} The allocation of banks for each tensor~(3/4) for 2 levels of on-chip memory hierarchy. (6/8 attributes.)
    % \chris{what do you mean by 2 memory hierarchies?}
\end{enumerate}

These attributes induce a map space that is too large to exhaustively search.
For example, the map space size for the ResNet Conv\_4 layer~(CNN-Layer) is $\approx10^{25}$ valid mappings.

To characterize the search space, we sampled 1~M samples from each of the map spaces implied by Table~\ref{tab:problem_shapes} and computed the energy of each sample, which resulted in a $(mean, std)$ of $(44.2,231.4)$, $(48.0,51.2)$ for CNN-Layer/MTTKRP respectively, when energy 
was normalized to a theoretical lower-bound energy for the given problem.
% \kartik{Get more stats: see the lowest 1\%. This should tell that there are very few mappings with low energy.} \chris{this para could use a punchline.  When you add one, ping me and I will check it.}

%\chris{this section is not consistent with mapping space terminology.  The mapping space only consists of valid mappings.  It sounds like what you mean above is the Cartesian product of programmable attribute settings.}
%\chris{Also, mapping space size depends on the specific problem.  Above, you simply give a single Mapping Space size for all problems in CNN-Layer.  What is going on here?}\kartik{Fixed, specified the exact problem. Although they are not all that different in size (order of 1 difference, max)}

\subsection{Search Methods and Comparison Metrics}
\label{subsec:eval:methods}
We compare Mind Mappings with following popular search methods used in prior work.
\begin{enumerate}
    \item \textbf{Algorithmic Minimum:} Refers to the theoretical lower-bound, possibly unachievable.
    \item \textbf{Simulated Annealing~(SA):} A popular black-box optimization method~\cite{simanneal}.
    \item \textbf{Genetic Algorithms~(GA):} Another popular black-box optimizer that uses evolutionary learning~\cite{genetic}.
    \item \textbf{Reinforcement Learning~(RL):} A popular unsupervised learning approach.
    \item \textbf{Mind Mappings~(MM):} This paper.
\end{enumerate}
We elaborate on how we implement each search method in Appendix~\ref{appendix:comparison}.

Two key metrics to judge a search method's effectiveness are the number of steps and amount of time needed to obtain an optimal solution.
Accordingly, we compare Mind Mappings against the above methods on two key metrics:
\begin{enumerate}
    \item \textbf{Iso-iteration Search Quality:} All approaches are run for fixed number of cost function evaluations. In case of Mind Mappings, the cost function is the trained surrogate~(Phase 1), whereas the other approaches query the actual cost function~(timeloop).
    \item \textbf{Iso-time Search Quality:} All approaches are run until a fixed wall-clock time.
\end{enumerate}

\begin{figure*}[ht]
  \includegraphics[width=\textwidth]{ASPLOS CR/main_result/iso-time_results.png}
\caption{Iso-time comparison of various search methods compared to Mind Mappings (MM).  Note the x-axis is log scale.}
\label{fig:main_res_time}
\end{figure*}

\subsection{Surrogate Model}
\label{subsec:eval:surrogate}

As discussed in Section~\ref{subsec:func_approx}, we implement the surrogate as a Multi-Layer Perceptron DNN.
We run Phase 1 once for each target algorithm.
That is, one surrogate is trained for all CNN-Layer results and a second is trained and used for all MTTKRP results.
This shows how the surrogate generalizes across problems for a given algorithm.
We elaborate on the details of the surrogate model and the training procedure in Section~\ref{subsec:eval:sensitivity}.

%\chris{leaving the rest of the details for the sensitivity section is ok.  one question I want to know now: were the target problems accidentally included in the training set due to randomness?}\kartik{Possibly unlikely. We sample independently for each dimension, for example, $K$ is sampled anywhere from 32-512. All the dimensions coming together to match the exact layer, not sure.}

%We train a deep 
%\chris{deep is redundant with "multi-layer"?}
%Multi-Layer Perceptron network as the surrogate model to approximate the accelerator cost function~(Phase 1, Section~\ref{subsec:func_approx}).
%We train one MLP per algorithm-accelerator pair~(one each for CNN-layer and MTTKRP) for this evaluation to demonstrate the generalization of the MLP across the family of problems of each algorithm.

%\chris{The eval so far seems to be missing a key part of the methodology: how the surrogate is trained.  For example, in the reviews it wasn't even clear to the reviewers that 1 surrogate was trained for all of the DNN benchmarks and such a paragraph would clear that up.}
%\kartik{Problem is that there is a separate section on the sensitivity study, that has a lot of details on the surrogate. One possiblity is to bring it here, or the other is to point to that. }

\subsection{Comparing Mind Mappings to Black-Box Optimization Approaches}
%\chris{Not clear what iso-iteration means, since MM only calls the cost function during phase 1.}
%\chris{more general comment: we need to define the terms for what all schemes are doing more precisely, probably in S5.2.  I.e., that to perform an iteration of work, all schemes call a cost function, but that online, MM calls a different cost function (the surrogate).}\kartik{Fixed}
% \chris{these definitions are a bit confusing.  The distinction is simply that the x-axis is time vs. iterations, no?  That is providing more information than saying we run for a fixed time (which just refers to the max x-axis value).}

We plot iso-iteration and iso-time comparisons between Mind Mappings (MM) and the other search techniques~(Section~\ref{subsec:eval:methods}) for different problems~(Table~\ref{tab:problem_shapes}) in Figures~\ref{fig:main_res_iters} and \ref{fig:main_res_time}, respectively.
In both figures, the $y$-axis represents normalized EDP with respect to the algorithmic minimum for that problem~(Section~\ref{subsec:eval:methods}).
The $x$-axis represents iterations and time, respectively.
To isolate the effects of randomness, each method was run 100 times and the averaged results are plotted, i.e., for each iteration across the 100 runs, we average the EDP across the runs.
%\chris{the previous sentence screams error bars}\kartik{I have the data, but the figures get too clumsy. At 5000 iterations, the deviation is very small (~$10^{-2}$)}
%\chris{need to clarify how you calculate avg.  I.e., is it "for each iteration i across all 100 runs, take average" for iso-iteration?}\kartik{Correct, fixed}

\subsubsection{Iso-iteration Comparison.}
\label{subsubsec:iso_iteration}
Figure~\ref{fig:main_res_iters} shows iso-iteration comparisons for all the search methods for every target problem represented in Table~\ref{tab:problem_shapes}.
Overall, MM outperforms SA, GA, and RL with mappings that have $1.40\times$, $1.76\times$, and $1.29\times$ lower EDP respectively, on average.
% \chris{from what iteration are these results sampled from?}\kartik{Last iteration (5000th)}
Further, solutions proposed by MM are only $5.3\times$ away from the (possibly unachievable) algorithmic minimum.
MM has a distinct advantage in that it performs a guided search using the approximate gradients derived from the surrogate model, where gradients by definition point at the steepest descent.

For CNN-layer based problems, 
% \chris{CNN-Layer?}
MM converges to much better solutions compared to other approaches and does so within 1000 iterations.
The speed of convergence is the key characteristic that demonstrates the effectiveness of gradients and the guided nature of the search.
More importantly, MM performs well on every target problem~(layer shape for CNN-layer); 
indicating that the surrogate indeed generalizes and generates useful gradients across the family of problems associated with the target algorithm.
%pointing to the generalization of the surrogate model and generated gradients across the family of problems associated with an algorithm.

We note that for MTTKRP-based problems, MM converges to slightly better solutions compared to other approaches.
MTTKRP-based problems have much smaller map space sizes~($\approx10^{19}$ for MTTKRP\_0 vs. $\approx10^{25}$ for ResNet Conv\_4) and much lower variance in their EDP~(standard deviation of $51.2$ vs $231.4$ across a dataset of 1M samples; c.f. Section~\ref{sec:eval:map_spaces}), pointing to a possibly simpler mapping space search.
In such cases, black-box optimization approaches are competitive with MM in terms of iso-iteration search quality.
However, MM still provides good solutions much faster than other approaches in terms of iso-time search quality, as we will see in Section~\ref{subsubsec:iso_time}.
%\chris{This paragraph is not in sync with the MTTKRP results.  Discussing them in the below paragraph is too late.}\kartik{Fixed}

Other methods have known weaknesses, and sometimes map space search-specific weaknesses, that may be contributing to their lower search quality.
Specifically:
SA suffers from an inefficient traversal in the search space due to the unguided nature of search.
Not only is the performance of GA sensitive to the choice of initial population, but GA also heavily relies on an assumption that combining
two strong attributes in two mappings~(e.g., $m_d^i$ and $m_d^j$)
%\chris{mapping?}\kartik{No, programmable atttributes. In GA, you mate two mappings by combining their strengths}
together will make an individual~($m'$) stronger. 
However, this is not necessarily
true in mapping space search.
For example, a good tiling for one loop order may not do well when combined with another loop order.
RL performs well compared to other black-box approaches, thanks to its superior heuristics using the actor-critic model based on deep deterministic policy gradient~(DDPG)~\cite{ddpg}.

%\chris{what is RL's weakness?}\kartik{Not as good as MM, and takes longer per step}

%\chris{what is the Figure 4-specific insight in this paragraph?  The above text just seem to be reiterating the known and already stated weaknesses of the other search methods.}
%\kartik{Last paragraph is not an already known weakness, I think it puts the results into perspective.}

% We found that Bayesian Optimization procedure with underlying Gaussian Processes is significantly compute expensive~\cite{gp_expensive} compared to the evaluation of the black-box function itself; making BO a bad choice for this problem.
% BO especially gets expensive to evaluate after a few 100 iterations, hence we plotted only up to 250 iterations with days of simulation.
% Exploring faster variants of BO, such as sparse Gaussian Processes~\cite{sparse_gp}, is future work.
% BO starts with a prior belief and repeatedly samples from the search space to improve the confidence of the surrogate model, which is then used to predict good solutions.
% However, given the complexity and size of the search space, it is hard to develop an accurate generalized surrogate, limiting its ability to find optimal solutions.
% \todo{placeholder if RL simualtions are complete.}

%Finally, we note that solutions proposed by MM are only $5.3\times$ away from the algorithmic minimum,
%on average, pointing to the proximity to global optimum.
%The algorithmic minimum cost is possibly unachievable in practice, hence the global optimal should exist within this range.

% \chris{I moved the algo 5.3x minimum text to the first iso-iteration paragraph}

\begin{figure*}[t]
  \centering
  \subfloat[Training and test loss.]{
% 	\begin{minipage}[c][1\width]{
	   %0.24\textwidth}
	   \centering
        \includegraphics[width=0.30\textwidth]{main_result/overfit_analysis.png}
        % \vspace{-5mm}
        \label{fig:loss}
% 	\end{minipage}
	}
 \hfill 	
  \subfloat[Choosing a loss function.]{
% 	\begin{minipage}[c][1\width]{
	   %0.24\textwidth}
	   \centering
        \includegraphics[width=0.30\textwidth]{main_result/loss_function_analysis.png}
        \label{fig:compare_loss}
% 	\end{minipage}
    }
  \hfill
  \subfloat[Sensitivity to training set size.]{
% 	\begin{minipage}[c][0.95\width]{
	   %0.24\textwidth}
	   \centering
        \includegraphics[width=0.30\textwidth]{main_result//sensitivity_dataset_size.png}
        \label{fig:dataset_size}
% 	\end{minipage}
	}
\caption{Experiments to determine the DNN topology and the loss function.}
\label{fig:sensitivity_train}
\end{figure*}

\subsubsection{Iso-time Comparison}
\label{subsubsec:iso_time}
%An important metric in mapping space search methods is the time required to find the optimal solution.
%We now evaluate search methods in an iso-time study.
Figure~\ref{fig:main_res_time} performs an iso-time study by plotting time as the $x$-axis~(note the log scale) when all search methods are run on an Intel Xeon E5-2637 v4 CPU.
Overall, MM outperforms SA, GA, and RL by $3.16\times$, $4.19\times$, and $2.90\times$ respectively on iso-time metric when run MM is run until convergence~(62.5 seconds).
This is possible since MM does not need to query the expensive cost function~(timeloop) every step, unlike other approaches.
Instead, MM uses the surrogate model to predict meta-statistics at every step ~(Section~\ref{sec:method:output_rep}), which in turn generates gradients to guide the next step.

Accordingly, we find that MM is 153.7$\times$, 286.8$\times$, and 425.5$\times$ faster per step than SA, GA, and RL respectively.
With recent hardware/software advances in Deep Learning, the gap between MM and other approaches can further widen by using state-of-the-art infrastructure instead of a CPU, as in this evaluation.
%\chris{previous sentence: it is unclear whether we expect future improvements, or whether we are already reaping the benefits of DL infrastructure}\kartik{Both. It is already good, can be better if we use GPU.}
While RL outperforms SA/GA in iso-iteration search quality, the per step cost of RL is significantly higher than MM. 
%\kartik{RL is of course slower than MM, we want to say, it is slower than SA/GA too, but it does better than them in iso-iteration.}
To summarize: MM not only generates higher-quality mappings compared to other approaches, but generates those mappings faster. %, which is crucial for modern day compilers.

% While time per iteration may be influenced by the implementation of the library itself, we find that the majority of the time is spent on evaluating the cost.
% Figure~\ref{fig:exec_time} depicts the execution time per step for each of the evaluated methods, averaged over 250 steps.
% The bars also segregate the time spent on evaluating a mapping and the time spent on choosing the next step.
% Overall, Gradient search is 15.2$\times$, 12.7$\times$, and 32$\times$ faster per step than SA, GA, and BO respectively.
% drastically reduces for our surrogate model, compared to the actual cost model~(based on timeloop).
% This number can further increase by using modern hardware solutions for Deep Learning such as GPUs and ASICs.
% Additionally, 
% On average, the cost evaluation is 456.4$\times$ faster 
% \chris{does that match the 19x figure from the rebuttal?}
% than the cost model~(Timeloop) with MM, thanks to much simpler matrix multiplication operation of the DNN inference.
% \chris{above paras are pretty rough writing wise and need a pass}

\textbf{Using Surrogate Models for Black-box Approaches.} We note that it is possible to improve traditional black-box methods in terms of time-per-step by using a surrogate, as explored in a several prior works~\cite{ithemal, tvm, release}~(refer to Section~\ref{subsec:surrogate_related}).
While such surrogates are not beneficial in finding better mappings (i.e., will not improve iso-iteration search quality), they enable more cost function queries per unit time, which improves iso-time search quality.
%However, errors in the surrogate's prediction can hamper search quality, as black-box methods develop heuristics based on the previous samples seen during the search to make moves in the search space.
%In this paper, we propose to use a meta-statistics based cost representation~(Section \ref{sec:method:output_rep}) to train the surrogate model that can reduce the error with respect to the ground truth.
%\chris{it isn't clear what the last two sentences are saying.  It sounds like you are saying there is a fundamental issue with training high-quality surrogates as proposed by the other methods, which seems dubious unless you can point to previous papers.}
%\kartik{I am not really sure what to say in this section (which the shepherd wanted so badly). What I am trying to communicate is that, Yes you could use a suroogate model for b-box approaches, but it won't make you better in iso-iteration, but will help in iso-time. Also, if the surrogate has errors, it would compound over the run, as bbox methods generate heuristics during run time. Can we discuss once?}


\subsubsection{Summary}

Overall, we note four key takeaways:

\begin{enumerate}
    \item \textbf{Generality:} Mind Mappings generalizes over different algorithms, architectures, and target problems, as demonstrated by the search performance.
    %\chris{what is the third metric?}\kartik{Three metrics was a bug. Should the sentence need anything more? I don;t want to make it verbose}
    \item \textbf{Quality of Solution:} Mind Mappings finds better/as good mappings compared to other popular methods.
    \item \textbf{Optimality:} The Mind Mappings returns mappings that are within $5.3\times$ of the possibly unachievable lower bound, suggesting they are close to the achievable global optimum.
    \item \textbf{Time per Step:} Mind Mappings uses a surrogate model instead of the (expensive) accelerator cost function at every step, allowing it to perform more steps per unit time relative to other methods.
\end{enumerate}

\subsection{Surrogate Model} 
\label{subsec:eval:sensitivity}

We now provide details for the MLP used as the surrogate, and show sensitivity studies used to determine the MLP's training procedure and architecture.

\textbf{Input and Output Vectors.} 
The input mapping vector is 62/40 values in length for CNN-Layer/MTTKRP, respectively, which includes the representation of the problem id, tile sizes, parallelism, loop ordering, and buffer allocations.
We elaborate on the input vector representation for CNN-layer below.
\begin{enumerate}
    \item \textbf{Problem ID~($p_{id}$):} $P_0 = \mathbb{Z}^7$: a 7-tuple indicating the problem shape~($N,K,C,H,W,R,S$; see Table~\ref{tab:problem_shapes}).
    \item \textbf{Tile Sizes:} $P_1 = \mathbb{R}^{21}$: a 21-tuple representing what factor larger each tile dimension is relative to the corresponding dimension in the next level of the memory hierarchy (e.g., $R_c$ in the 1D-Conv tiled example in Code~\ref{code:tiled}).
    There are 21 factors, for the 7 dimensions in the 3-level memory hierarchy. 
    \item \textbf{Parallelism:} $P_2 = \mathbb{Z}^7$: a 7-tuple to indicate the degree of spatial parallelism for each dimension.
    Spatial parallelism is represented in terms of a factor for each dimension, similar to how tile sizes are represented (above).
    %For example, if the for loop on Line 2, Code~\ref{code:untiled}, is parallelized, parallelism in $R$ dimension is the shape of $R$) per dimension.
    %\chris{????????????????}
    \item \textbf{Loop Order:} $P_3 = \mathbb{Z}^{21}$: a 21-tuple indicating the loop order, represented as a permutation of the 21 (7 dimensions times 3 levels of memory) loops.
    For example, in 1D-Conv $W\rightarrow R$ is represented as $[0,1]$, and $R\rightarrow W$ is $1,0$.
    \item \textbf{Buffer Allocation:} $P_4 = \mathbb{R}^6$: a 6-tuple indicating the percentage of banks in each of the 2 levels of on-chip memory allocated to each of the 3 tensors~($\inp$, $\out$, and $\filt$ in Equation~\ref{eq:conv2d}).
\end{enumerate}

The output cost vector has 12/15 neurons for CNN-Layer and MTTKRP, respectively. 
Each neuron represents the energy spent in accessing a specific level of the memory hierarchy~(3) for each input/output tensor~(3/4), overall energy, compute utilization, and overall cycles for execution.
Inputs and outputs are normalized over the dataset to have a mean of 0 and standard deviation of 1, as discussed in Section~\ref{subsec:func_approx}.

\textbf{DNN Topology and Training.}
We choose a 9-layer deep MLP with \lstinline{[64,256,1024,2048,2048,1024,256,64,12/15]} neurons in each layer for CNN-Layer/MTTKRP, respectively, as the surrogate model based on a grid search.
% Figure~\ref{fig:number_layers} depicts a sensitivity study where we add 2048-neuron layers on top of the baseline 9-layer MLP.
%of the DNN by adding hidden layers with 2048 neurons to the network.
% Adding layers after 9 does not improve solution quality, so we retain the 9-layer MLP architecture.
% \chris{what about <= 8 layers???  Why is 9 necessary?}\kartik{Yeah, I did not try below 9, which seems like a missing point in grid search. }
We train the MLP for 100 epochs with a learning rate of $10^{-2}$, which is decayed by a factor of 0.1 every 25 epochs, and a batch size of 128.
We use the Stochastic Gradient Descent (SGD) optimizer with a momentum value of 0.9.
Loss over the training duration is depicted in Figure~\ref{fig:loss}.
The MLP converges at around 60 epochs, and the test loss closely follows the train loss, indicating that we do not overfit.
 
\textbf{Dataset.}
We train the model with 10~M samples drawn with uniform random probability from the space of representative problems associated with the target algorithm~(Section~\ref{sec:method}).
%\chris{what does representative mean?  it is important they do not include the target problems.  from the description below, it sounds like you just sample randomly from the universe of problems.  If so, don't say the word "representative".}\kartik{Correct, updated the sentence.}\chris{still isn't clear.}
``Representative problems'' means we sample from a range of typical values for each parameter making up the problem~(e.g., the $N,K,C,H,W,R,S$ dimensions for CNN-layer). %\kartik{We should not use hyperparameter, dimension size, shape etc are probably better}
For example, we randomly sample the value of $K$ for CNN-layer from the range \lstinline{[32,512]}, which should cover the typical range of $K$ in practice~\cite{Resnet,vgg,Alexnet}.
That Mind Mappings performs well given this methodology suggests that the surrogate is able to interpolate and predict costs for unseen combinations of problem parameters. %\kartik{Problem shape, as used in S2}
Figure~\ref{fig:dataset_size} compares the search performance on surrogate models trained with 1~M, 2~M, 5~M, and 10~M samples.
While the datasets with more than 5~M samples lead to a well-trained model for this problem, surrogates used for the evaluation were trained with 10~M samples.
We note that, even when the dataset size is smaller than 5~M, search quality is not significantly hampered.
%We leave a detailed study of smaller training set sizes to future work.

% \chris{uh.  how small can we go before we fall off a cliff?  why didn't we evaluate this?}\kartik{Yes, a hole in evaluation. Should we remove this graph, because it is not helping. Possibly, we are underselling.} 
% \chris{I think it is ok to leave in as is.  But it is a shame we didn't do the study.}

\textbf{Loss Function Choice.} We use the \emph{Huber} loss~\cite{huber} function as the loss criterion for training with the SGD optimizer.
%\chris{I can't parse "... the training clubbed ..."}\kartik{rephrased}
Figure~\ref{fig:compare_loss} compares the performance of several popular loss functions used in regression such as the \emph{Mean Squared Error}~(MSE) and \emph{Mean Absolute Error}~(MAE).
Interestingly, MSE loss, a widely popular loss function used in regression problems, performs poorly in our setting.
We attribute this to the fact that MSE greatly punishes outliers, leading to a large variance in loss and instability in training.
By contrast, \emph{mean absolute error} punishes small variations, leading to sub-par performance.
Huber loss is similar to MSE when variations are small and is similar to MAE when the variations are larger, thus creating a good balance between the two loss functions.

\textbf{Model size.} When weights are represented as 32~bit floats, the surrogate model takes 35~MB of storage.
With recent advances in pruning and quantization~\cite{deepcompression, eie}, the model can be likely be compressed significantly.
Therefore, we believe that model size should not be a constraint in adopting Mind Mappings for real world applications.





==> intro.tex <==
\section{Introduction}
\label{sec:intro}

The compound effect of the slowing of Moore's law coupled with a growing demand for efficient compute has ushered in an era of specialized hardware architectures.
Due to their inherent performance, energy, and area characteristics, these accelerators are driving innovation in diverse areas such as machine learning~\cite{eyeriss, ucnn, cnvlutin, eie, scnn, tpu}, medicine~\cite{medical1, medical2, medical3}, cryptography~\cite{crypt1, crypt2}, etc.
% \chris{polish to remove duplicate 'further'.  This sentence can still connect better to next para.}
% To push the benefits further, 
They are seeing a wide variety of deployments ranging from cloud to edge---forcing designers to make complex design decisions to achieve their efficiency objectives.
%Given the significant power and per-formance efficiency that specialized hardware solutions canprovide, they are
%\chris{I removed emph from the word accelerator.  emph should be reserved for terminology, and sparingly used to emphasize o/w important words.  accelerator does not reach the bar imo.}
%These specialized architectures are often implemented as accelerators within an on-chip system. 
% These accelerators are deployed in variety of target scenarios---from edge to cloud---forcing designers to make complex design decisions to achieve their performance and efficiency objectives.

Although they are specialized, accelerators are often flexible~\cite{maeri, dna, morph, flexiflow, eyerissv2}, designed to support different parameterizations of a single algorithm to even a range of algorithms within or across domains.
This flexibility forces architects to decouple the act of designing the architecture from the act of mapping a specific \emph{problem}--a parameterized instance of an algorithm--onto the architecture.
This is shown in Figure~\ref{fig:design_process}.
First, pre-fabrication, architects 
choose architectural parameters to suit the budget and deployment requirements of expected target problems---a process referred to as \emph{Architecture Design Space Search}. 
This can include decisions such as the number of processing elements, on-chip buffer sizes, network-on-chip topology, bandwidth to off-chip memory, etc.
Second, post-fabrication and based on the designed-in flexibility of the hardware, 
architects or users map target algorithms to the hardware---referred to as \emph{Mapping Space Search}.
These decisions can include choosing how much of each buffer to allocate for each data structure,
mapping of computations to processing elements, etc., and are analogous to writing/compiling programs for general-purpose processors.

\begin{figure}[t]
\begin{centering}
  \includegraphics[width=0.85\columnwidth]{figures/design_process_new.pdf}
  \caption{Architecture design and algorithm mapping in hardware accelerators.
%   \chris{should be "mapping space search}
  %\chris{Relatively minor, but I don't like the color scheme.  It makes the figure look powerpoint generated, which makes it look cheap.}
  }
  \label{fig:design_process}
\end{centering}
\end{figure}
  
Mapping space search is an important problem, and currently faces severe scalability and performance challenges.
To start, prior work has shown that problem efficiency is very sensitive to the choice of mapping~\cite{eyeriss, scnn, morph, timeloop, maeri, flexiflow, dna}.
Further, the same studies illustrate how optimal mapping varies significantly depending on problem size and parameters (e.g., DNN model parameters), resource availability, performance and power requirements, etc.
This suggests that mapping space search will constitute an increasing recurring cost, as accelerators are re-targeted for new problems.

Making matters worse, simply gaining intuition for how to search through the map space, or how to pose the search to an automated tool, is an ad-hoc and expert-driven process.
Accelerators lack consistent hardware-software abstractions, such as instruction set architectures (ISAs) in the general-purpose computing world, and instead rely on bespoke configurable hardware components designed to provide higher degrees of control and efficiency.
% as depicted by Figure~\ref{fig:intro_motivation}.
% \chris{I don't think this figure is adding anything here.  And, again, it is giving me more of a feeling of homogeneits than lack of consistent interfaces b/c each accelerator is a set of knobs.}
Further, different accelerators tend to have different degrees of configurability in different hardware components, ranging from programmable networks on chip~\cite{maeri}, buffers~\cite{buffets,morph}, address generators~\cite{ganax}, etc.
While this may be suitable for experts with deep knowledge of both the architecture and algorithm, it clearly does not scale to non-experts programming new hardware with new algorithms.

% \chris{insert the comment on halide/timeloop requiring a custom DSL somewhere in previous para.  reproduced below:}
% \angshu{Prior work[Timeloop,Halide Autotuner/ASPLOS] has attempted to address the scalability problem by requiring users to describe their architecture using a DSL to instantiate a restrictive template. Their tools will generate a mapper for an architecture that can be expressed using that template, but not otherwise.}

%%- expensive
%%  * no good search tools
%%  * recurring cost
%%- important
%%  * prior work has shown it is important
%%- not scalabe
%%  * requires expert knowledge

Making matters even worse, while prior work has proposed tools and algorithms (i.e., \emph{Mappers}) for automatically searching the map space, all existing approaches have serious limitations due to search space complexity~\cite{morph,timeloop,tvm, release, flextensor}.
% \chris{there are some others pointed out in the isca reviews we should cite}
%the map space implied by these bespoke configurable units creates a notoriously difficult search problem.
First, the search space is often high dimensional~(i.e., each degree of configurability induces a dimension), causing a combinatorial explosion of possible mappings and rendering exhaustive techniques ineffective~\cite{timeloop}.
Second, the search space is both non-convex (many local minima) and non-smooth (not differentiable), forcing prior work to rely on \emph{black-box optimization}~\cite{blackbox} approaches. % that results in reduced search quality and higher cost.

To summarize, while configurable accelerators have demonstrated their potential, the lack of an efficient and high-quality Mapper hinders broader adoption.

%\textcolor{red}{Specifically, given a non-smooth search space, %black-box optimization-based mappers have to either randomly pick %candidate configurations or based on some heuristics learnt from %prior samples, and keep the one that maximally improves a cost %function ($C$), and ignore others.
%This method makes the search quality depend on the number of %attempts one can afford, and the search cost is still proportional %to the overall size of the search space.}

% Black-box optimization is fundamentally a trade-off between search quality and cost.
% Specifically, black-box optimizers can only make decisions based on observing the cost of optimizer-selected candidate mappings.
% The more times the cost function is evaluated, the better the guarantee of a result closer to the optimum.

%\chris{
%Suggested text for above paragraph:
%
%Specifically, search algorithms `walk' through the search space by %iteratively calling
%\[\theta = \argmin_{\theta'\in\mathsf{neighbors(\theta)}} %C(\theta')\]
%where $C$ is the cost function and $\theta$ is the current %configuration.
%We call the $\argmin$ operation \emph{local-neighborhood search}.
%Black-box optimizers use heuristics or brute-force methods to %implement local-neighborhood search, resulting in either a %sub-optimal walk through the search space and/or high search time.
%}

% \begin{figure}[t]
% \begin{centering}
% \includegraphics[width=0.9\columnwidth]{figures/intro_motivation.pdf}
% \caption{\small Lack of consistent hardware-software abstraction for accelerators makes it hard to perform a mapping space search.}
% \label{fig:intro_motivation}
% \end{centering}
% \end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW DRAFT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{This Work}

This paper addresses the challenges above by proposing \emph{Mind Mappings}, a scalable and automated method to quickly and effectively perform mapping space search.

As mentioned previously, the key challenge hindering prior work is that mapping search space is non-smooth, forcing prior work to resort to black-box optimization techniques.
This is because the accelerator \emph{cost function}---which search algorithms use to evaluate the cost of a given candidate mapping---is non-smooth.
For example, the cost function might be an architectural simulator or the accelerator itself.

Mind Mappings addresses this challenge by constructing 
a \emph{differentiable} approximation of the cost function, called the \emph{surrogate}~\cite{surrogate_definition, surrogate_definition_0, surrogate_definition_1}.
Using the surrogate, Mind Mappings derives gradients for the cost function, with respect to candidate mappings, and uses those gradients to perform
a powerful first-order optimization technique, Gradient Descent~\cite{backprop, efficient_backprop}, to quickly find low-cost mappings.

The key insight here is that the differentiable surrogate of the actual non-differentiable cost function can provide us with approximate gradients, which are sufficient to guide the search along the direction of steepest descent, even in the absence of true gradients.
This insight simultaneously improves map space search quality and reduces map space search time, as gradients by definition point in the direction of the greatest reduction in cost.

Crucially, Mind Mappings formulates both predicting the cost of a mapping and finding the optimal mapping as \emph{learning} problems, thereby doing away with requiring expert knowledge in the target domain.
% Only the mapping and cost vectors to the surrogate model need to change for a different choice of accelerator or algorithm.


%Such a differentiable approximation not only allows us to obtain \emph{gradients}, where gradients represent the relative benefit of a change in the mapping, but also helps avoid the need to query the computationally expensive cost function every step~\cite{tvm, ithemal, release}\todo{Cite more}.
%Importantly, \emph{the surrogate need only be constructed once (offline)} for a given algorithm and accelerator, amortizing its cost over multiple mapping space searches.

%Second, with access to the gradients via the surrogate, Mind Mappings uses 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% </NEW DRAFT>
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\begin{comment}
\subsection{This work}

\kartik{LOCKED Chris/Kartik}
\chris{we still need to converge on how to present the contribution, in light of the work difftune cites}

% \chris{based on current text in 1.0, need to echo these 3 points:
% * mapping is important, and changes per problem
% * hard to derive mapper for a new architecture
% * once mapper is derived, space is hard to search
% }
To address the challenges above, this paper proposes a scalable and automated method to quickly and effectively perform mapping space search.
\emph{The key idea is to approximate the search space with a differentiable surrogate function, thereby turning what was a non-differentiable search space into a differentiable search space.}
\chris{this is not the best articulation of the main idea.  just because I have a differentiable surrogate doesn't imply that I use it to pose the problem as white box}
By building a differentiable approximation of the search space, we turn mapping space search into a \emph{white-box optimization problem},
where the mapper performs a \emph{guided-search} based on \emph{gradients}
(i.e., the relative benefit of a change in mapping, $\frac{\Delta C}{\Delta M}$, where $\Delta C$ is the change in cost, $\Delta M$ is the change in mapping vector).
% of the current mapping $K_1$ to find the next mapping $K_2$.
This insight drastically reduces the search cost and improves the search quality, as gradients by definition point in the direction of the greatest reduction in cost.

\chris{greatest local reduction in cost.  need to make how this fits into the overall search more clear.}

In more detail, our method is a two step procedure:

\noindent\textbf{Smooth function approximation.}
First, we approximate the otherwise non-smooth complex search space with a smooth, differentiable surrogate.
% \chris{saying gradients here is too early.  I think this next sentence can be removed.}\kartik{I think it is okay, let the readers register it as they go to step 2}
This not only enables us to generate gradients, but also helps avoid the need to query the computationally expensive cost function every step.
% Unlike black-box search methods, gradients enable our search to immediately determine the best next move, because gradients by definition point in the direction of the greatest improvement in loss.
% A differentiable function not only is fast to build, but also allows us to quickly search through candidate mappings.
Importantly, \emph{the surrogate need only be constructed once (offline)} for a given algorithm and accelerator, amortizing its cost over multiple map-space searches.
% i.e., not once for every candidate mapping.
%Thus, surrogate can be constructed offline, thereby amortizing the cost of training the surrogate.

% \begin{figure}[t]
% \begin{centering}
%   \includegraphics[width=0.9\columnwidth]{ASPLOS/figures/search_methods_compare.pdf}
% \caption{\small Comparing MM approach to black-box optimizers. $K_i\in K$ where $K_i$ is a distinct configuration setting of the accelerator, $C$ is the accelerator cost function, and $|K|$ is the size of map space.
%   }
% %   \vspace{-4mm}
%   \label{fig:search_description}
% \end{centering}
% \end{figure}

\noindent\textbf{Searching over the smooth function.}
Second, we make a key observation that the smooth surrogate can be used to \emph{directly} generate a move in the mapping space, relative to a reference mapping, \emph{that will maximally reduce cost} given C.
Consider an analogy to deep learning.
In deep learning back-propagation is used to, given an input, generate gradients to train model parameters.
In our setting, we have a fixed model (the surrogate) and use back-propagation to \emph{train the input (mapping)}.
%based on the key observation that the trained surrogate model can not only predict the cost given a configuration~(forward pass), but can also generate the change needed in the current configuration to steer it towards a target cost C~(backward pass).
%Given the differentiability of the surrogate, we achieve this goal efficiently using gradient descent via back-propagation, also a key enabler in modern deep learning approaches.
To find an optimal mapping, we construct a theoretical lower-bound cost and perform multiple iterations of back-propagation, each of which incrementally evolve an initial (random) mapping to a more optimal mapping. 
%Starting with a random mapping, we iteratively update that mapping while keeping the surrogate model fixed.
%This enables us to perform efficient guided search in the search space.
% Second, we use gradients generated from the approximated cost function to iteratively update the current mapping towards an better one.
%There are two challenges. %involved in this.
%\chris{not clear what way would be ``straightforward''.  it would help to define a strawman and illustrate why it doesn't work.}
% The idea is inspired by techniques used in adversarial machine learning~\cite{adversary_0,adversary_1}. 

% While we do not know the global optimal cost, it is sufficient to generate gradients based on what will push the cost closer towards a desired value.
% We construct a 
% This is straightforward, e.g., the lower the cost the better.
%possibly un-achievable value, e.g., ``zero cost.''
%\angshu{Moving towards zero cost seems to be a natural thing to do. I suppose what complicates things is that the cost itself is a feature vector, and the optimal solution may not be "less-than" a suboptimal solution for each element in the vector. Thus, attempts to move towards an all-zeroes optimal cost vector may lead the search on a wild goose chase.}
%\chris{interesting you bring this up.  see a comment by me before which is now commented out in the latex :).  I may have jumped the gun a bit on changing it to zero cost.}

%we use an \emph{oracle} cost, which represents the theoretical lower bound of the possible cost of execution to guide the search.
%\chris{what happens if you choose a too-ideal oracle cost, e.g., 0?  is the technique less effective?} \kartik{When I experimented earlier, it didn't change much. I will need to reverify.}



% that : not every single input in the mapping space is uniquely mapped to an output cost.
% \chris{the cost function is many to one?}
% In other words, the search space is not as complex as the number of possible mappings in the map space might make us believe.
% \chris{not clear what you mean by a function approximation.  a new function f' which is a bijection with the cost space?}
% Therefore, one can perform a \emph{function approximation} of the algorithm-hardware interaction for every mapping that significantly simplifies the search.
% \chris{I have no intuition about how much this simplifies the search space.  why do you claim the original cost function is many to one in the first place?  do we have evidense of this?}
% Additionally, choosing a differentiable function approximator, such as linear combination of parameters or neural networks, can enable us to get gradients of the cost function, vastly improving the efficiency of the search by performing a guided exploration.
% \chris{my sense is still that this last sentence is the key peice ... but I could be wrong}

% Recent advances in machine learning have been powered by gradient descent based methods, where the parameters are iteratively updated based on the gradients.
% Given the effectiveness of gradients in these problems, we explore the feasibility of gradient descent based search methods in algorithm-accelerator mapping space search.
% This is particularly challenging due to the non-smooth, non-differentiable nature of cost functions associated with hardware accelerators.
% Additionally, unlike in typical classification setting where the problem statement is to predict the output class for a given input, this problem requires finding a good input that minimizes the output, as shown in Equation \ref{eq:schedule}.

Not only is this process efficient (as it chooses good moves in $O(1)$ steps), it also does not require expert knowledge in the target domain.
Because, both predicting the cost given a mapping, and finding an optimal mapping given a lower-bound cost, are formulated as \emph{learning} problems.
Only the mapping and cost vectors to the surrogate model need to change for a different choice of accelerator or algorithm.



% The accelerator is simply represented as a set of features which can be changed to generate mappings, and an algorithm-agnostic cost function returns a cost given a mapping.

%we leverage machine learning to \emph{learn} the approximated model.
%\chris{grammar issues in next sentence:}
%By casting each algorithm-accelerator map space as a learning problem we do away with expert heuristics, thereby improving the scalability of the search method.
% which makes our method scalable across accelerators. \todo{Develop this paragraph for scalability}
\end{comment}

%Based on the above ideas, we develop a whitebox optimizer for algorithm-accelerator mapping problem using a deep neural network~(DNN) trained with back-propagation as the cost function approximator.
% First, we approximate the cost function using a deep neural network, which can effectively capture the non-linearity of the cost function and provide differentiability.
% Then we use the approximated differentiable cost function to get gradients to perform an efficient traversal in the search space.
This paper makes the following contributions:
\begin{enumerate}
    \item  To the best of our knowledge, 
    our work is the first to enable 
    %ours is the first work to design a framework for 
    \textit{target domain-independent} mapping space search for programmable accelerators. 
    We require neither expert knowledge in the target application domain(s), nor any domain specific heuristics for handling programmable hardware attributes.
    % \item To the best of our knowledge, ours is the first work to focus on a comprehensive study of crucial algorithm-accelerator mapping space search problem and take steps towards developing efficient search methods for the same.
    % % \chris{what would TVM say about this?}\kartik{TVM does not focus on the search problem. Is this claim unnecessary?}
    % \item We formulate and formally define the mapping space search problem.
    \item To the best of our knowledge, 
    our work is the first to formulate mapping space search as a first-order optimization problem, enabling an efficient  gradient-based search that is able to quickly find high-quality mappings.
    %The key idea is to build a smooth cost function approximation, and to use that function to incrementally \emph{evolve an input mapping into a more optimal mapping}.
    %Crucially, each move in the search space maximally reduces cost and only requires $O(1)$ queries to the cost function.
    %We develop a new method to efficiently find high-quality mappings based on cost function approximation and gradient-based search.
    %training procedure to train a surrogate model of the hardware accelerator using deep neural networks to get a smooth, differentiable approximation of the cost function.
    %\chris{I would, again, advise to combine these two (this and next one) contributions and discuss things more generally.  ``We develop a novel gradient-basedsearch method based on the ideas of smooth function approximation and mapping refinement based on an oracle cost.}
    %\item We propose an algorithm to generate gradients to a valid mapping vector that iteratively updates the mapping vector to minimize the execution cost.
    \item 
    We extensively evaluate Mind Mappings across two target algorithms---CNNs and MTTKRP---comparing against multiple baseline search heuristics including simulated annealing (SA), genetic algorithms (GA), and reinforcement learning (RL).
    For CNNs and MTTKRP, the proposed search method finds mappings with an average $1.40\times$, $1.76\times$, and $1.29\times$ (when run for a fixed number of steps) and $3.16\times$, $4.19\times$, and $2.90\times$ (when run for  a fixed amount of time) better energy-delay product over SA, GA, and RL, respectively. 
    % Also, the proposed gradient search is only $5.32\times$ the possibly unachievable theoretical lower-bound, indicating proximity to the global minima.
    \item To facilitate further adoption, we provide a reference implementation of the Mind Mappings framework here: \url{https://github.com/kartik-hegde/mindmappings}.
\end{enumerate}

% The rest of the paper is organized as follows.
% Section~\ref{sec:mapspace} develops a formal definition of the algorithm-accelerator search problem.
% Section~\ref{sec:blackbox} gives background on existing methods for black-box search.
% Section~\ref{sec:method} describes the proposed method.
% Section~\ref{sec:eval} evaluates the proposed method on a CNN hardware accelerator and compares to existing methods.
% Finally, Section~\ref{Section~\ref{sec:conclusion} concludes

%We build an end-to-end infrastructure to evaluate the proposed approach for algorithm-accelerator map space search.
%To facilitate a wider adoption, we will open-source our toolflow if the paper is accepted. 
% We first 

% The key contribution is developing a technique to obtain gradients for mapping decisions with respect to a target cost, steering mappings gradually towards a better one.

% % We train a surrogate model to approximate the otherwise non-differentiable accelerator cost function to a smooth, differentiable function.
% % The key idea is to then freeze the surrogate model, and get gradients to a randomly initialized input mapping vector to guide it towards an oracle cost.
% When evaluated on a CNN-based hardware accelerator, the proposed method produc    es upto $xxx \times$~(average) cost efficient mapping compared to simulated annealing.

% % We train a surrogate cost model of the hardware accelerator to approximate the otherwise non-differentiable cost function to a smooth, differentiable function.
% % Taking a cue from adverserial machine learning, we use the trained surrogate cost model to get gradients to inputs.


% % These mapping hyper-parameters may be deduced (1) in \emph{design-time} to be built into the hardware, or (2) in \emph{compile-time} to be mapped to the hardware, or (3) in \emph{run-time} to dynamically to mapped to the hardware.
% % In any of these scenarios, 

==> mapspace.tex <==
\section{Background}
\label{sec:mapspace}

%\chris{CHRIS HAS LOCK.  Working to address my own comments :)}

% \chris{looks like there is a latex typo above -- see two label references back to back.  move \ref{sec:mapspace} to the example sub-section?}

In this section, we formally define the algorithm-accelerator mapping space search problem and elaborate with an example.

%\angshu{A general concern I have throughout this section is the definition of an "application" (and consequently, "application specific hardware"). Which of the following is an example of an application: (a) a 7-deep affine loop nest, (b) a PQRSCKN loop nest (CNN layer) with loop bounds left unspecified, or (c) a specific CNN layer with PQRSCKN set to specific values (e.g., ResNet layer X)? I believe most of the definitions in this section only hold for definition (c). Otherwise, the mapspace itself is a function of *both* the architecture as well as the attributes of the problem/application that are left un-specified.}

%\chris{when you say (a) I assume you mean a completely un-specified nest?  IE any PQRetc?.  I think it is c.  Two things: (a) we only consider applications where the cost function is input-oblivious (see last para before B).  This may come too fast, but that implies things like loop bounds must be specified.  E.g., if we think of the mapping as the program, there is ambiguity about how much is hard-coded into the program vs. dynamic in the input.  But if we say we are input-oblivious that simplifies things: the cost cannot change with input, so the only option is for loop bounds to be included in the mapping.  This captures what we think of as config time.}

%\angshu{Absolutely I agree that loop bounds should be included in the mapping. What I'm asking is -- what is the space of legal mappings, and is it ... I'm stumbling on a word here ... "input" dependent. For example. I create a CNN accelerator. Of course I'm not going to create a ResNet Layer 4 accelerator. No, I think that may be an excellent thing to do instead of conversing over Overleaf :p} LMK if oyu don't see invite

\begin{comment}
\subsection{Design Process of an Accelerator}

\chris{a little repetitive given 2C}
The hardware-software design process depicted in Figure~\ref{fig:design_process} can be formally represented as a two step optimization problem represented in Equation~\ref{eq:minimize}.
\begin{equation}
\displaystyle{\minimize_{a\in A} \ \minimize_{m\in M_a} \ f(a,m)}
\label{eq:minimize}
\end{equation}
where each architecture $a$ in the set of all the possible architectures $A$ has a mapping space $M_a$ and the cost function $f: M\times A \mapsto C$ associates mappings for each architecture $m_a\in M_a$ to their cost in $C$. 
(We assume $C=\mathbb{R}$.)%the set of all possible costs $C$.
\end{comment}

%\chris{there is an assumption here that the algorithm is data oblivious.  I.e., this wouldn't work for a sparse architecture.  best to say this, and to give examples for what types of algorithm parameters are included in $m$, e.g., hyper-params.}

% \chris{it isn't very clear what is a mapping.  is m a program and its inputs, or just a program?  there is some subtlety here.  the programs you have been considering have input-independent DCFGs, hence input isn't important.  but generally, input is important.}

%Selecting an architecture $a\in A$ is done at design time (pre-fabrication).

\subsection{Algorithm-Accelerator Mapping Space}
\label{subsec:mapspace_search}

%\begin{figure}[h]
%\begin{centering}
%  \includegraphics[width=0.75\columnwidt%h]{figures/mapping_intuition.pdf}
%  \caption{\small Design Space for %Specialized Hardware Design. %\kartik{Improve further, ask Chris})}
%  \vspace{-.1pt}
%  \label{fig:accelerator}
%\end{centering}
%\end{figure}

In this paper, we assume that a hardware accelerator $a$ and a target problem $p$ is given, where a \emph{problem} is a parameterized instance of an algorithm.
For example, if matrix multiplication is the target algorithm, an example target problem is a matrix multiplication between two matrices of fixed shape (dimensions), 
irrespective of the contents of the matrices.
%\chris{shape is used a lot.  and deserves a more explicit definition.}\kartik{Shape is not used later in the paper any more.}
We begin by defining a mapping $m$ and the mapping space $M$.
\begin{definition}
\label{def:mapping}
\emph{Mapping.} A mapping $m \in P_0\times\dots\times P_{D-1}$ is a $D$-tuple, where $D$ is the number of programmable attributes of the given accelerator $a$.
Each element in the mapping vector, $m_d$ for $d\in[0, D)$ belongs to the domain of the $d$-th programmable attribute, $P_d$.
% \chris{value?}
% $m_d\in P_d$ is a value---which may be represented as an integer, string, or other encoding---in the domain of the $d$-th programmable attribute $P_d$. 
\end{definition}

\begin{definition}
\label{def:mapspace}
\emph{Mapping Space.} Given an \emph{accelerator} $a$ and a target \emph{problem} $p$,
we define a mapping space as
$$M_{a,p} = \{m \in P_0\times\dots\times P_{D-1}\;|\;a(m,i)==p(i)\;\forall i\in I_p\}$$ 
where $I_p$ denotes the possible inputs~(e.g., all possible matrices with a specific shape) to a problem $p$, $a(m,i)$ 
denotes the accelerator's output given mapping $m$ and input $i$, and $p(i)$ denotes the golden reference output given input $i$ for problem $p$.
\end{definition}

In other words, $M_{a,p}$ is the set of mappings that result in functional correctness for the given problem $p$ on the accelerator $a$.
We call such mappings \emph{valid} for $a$ and $p$ and write $M_{a,p}$ as $M$ for short when the context is clear.
%In other words, mapping space is the set of all mappings $m$ that result in functional correctness of the algorithm when executed on the architecture.
Intuitively, the different $m\in M$ can be thought of as different ``programs'' representing problem $p$ on accelerator $a$.
%\chris{another reason why $p$ as an input to $a$ seems redundant}
An example of a mapping space is given in Section~\ref{subsec:mapspace_example}.

With this in mind, the size of the mapping space varies based on the programmability of the underlying accelerator and the problem $p$.
On one extreme, the size of $M$ (denoted $|M|$) can be 1 for a fixed-function ASIC designed to execute one fixed problem.
In general, $|M|=O(\prod_{d\in[0,D)} |P_d|)$, where the number of attributes $D$ and the size of each attribute space $|P_d|$ is large.
%In other words, $|M|$ is exponential in $d$.
The Big-Oh captures how some mappings in the Cartesian product of assignments to programmable attributes may be invalid.
%\chris{This is a bit confusing since it is always $\prod_{i\in[0,d)} |P_i|$, it's just a matter of $d$ and how big each programmable attribute's domain is.  I think in the last part you are trying to bring out that in practice, map space size is usually $\ll \prod_{i\in[0,d)} |P_i|$ due to invalid mappings, but that is not coming out.}
%\kartik{Exactly, $d$ is a function of how programmable the accelerator is. The size of the domain of $P_d$ reduced due to invalid options is probably too complex to communicate here.}

\begin{comment}

%%%% floating text 

and focus on the inner optimization objective of mapping space search.
Hence, we will abbreviate $M_a$ and $m_a$ as $M$ and $m$ respectively.

The mapping $m$ is semantically the ``program,'' which is later provided an input $i$ which is unknown at mapping space search time.

\end{comment}
% \chris{suggestion: $m\in\{0, 1\}^D$, ie a vector of $D$ dimensions, where $D$ is the number of bits of programmable state in the accelerator.  
% Let $a(m, in)$ denote the accelerator running with mapping $m$ and input $in$.
% Let $p(in)$ represent a reference implementation for the algorithm, given the same input $in$.
% Then $M=\{m\in\{0,1\}^D\;|\;a(m, in)==p(in)\;\forall in\}$.

%CPUs can have an extremely large value of $d$\chris{practically infinite, actually.  only limited by the size of the address space}, representing all possible programs that implement a given algorithm.

% \begin{fallacy}
% All mapping decisions are non-architectural.
% \label{fallacy:mapspace}
% \end{fallacy}


% The outer optimization problem of architecture design space search is often heavily guided by the budgetary constraints such as area, while the inner optimization problem of mapping space search is dependent on the optimization.

\subsection{Mapping Space Search}
\label{subsec:map_space}

\emph{Mapping Space Search}
is the combinatorial search problem to find the mapping $m_{opt} \in M$ that minimizes the \emph{cost} $f$, where the cost function $f$ is the optimization objective set by the designer~(discussed further in Section~\ref{subsec:cost}).
That is,
\begin{equation}
m_{opt} = \argmin_{m\in M_{a, p}} f(a,m)
\label{eq:schedule}
\end{equation}
%\chris{again, why $p$ input to $f$.  $m$ is already derived from $p$.}

where the user specifies the problem $p$ and architecture $a$. %, which can be used to infer the mapping space $M$.
We denote $f(a,m)$ 
%\chris{ditto $p$ in $f$ issue}
as $f(m)$ for short. 
In theory, mapping space search can be performed at compile time or at run time. 
In practice, programmable accelerators today either perform the search completely offline, e.g., when compiling a new problem to the architecture~\cite{morph,maestro,scalesim}, or partly offline/partly online~\cite{nvdla}.
%\chris{why does nvdla do partly online?  since AFAIK it is dense only?}\kartik{Angshu/Po-An?}
%In practice,
%for typical programmable accelerators today, the search is usually performed offline, i.e., when compiling a new problem to the architecture~\cite{morph,maestro,scalesim}, or partly offline and partly when a new input arrives~\cite{nvdla}.

In this paper, we assume $f$ is a function of $a$ and $p$---not the problem input $i$.
%\chris{ditto $p$}
%This means that our methods apply to problems where mapping cost can be determined by looking at only the problem shape.
This holds for several important workloads, e.g., kernels in dense tensor algebra such as dense matrix multiplication and deep neural network training/inference~\cite{timeloop}.
However, it does not hold when input-dependent optimizations, e.g., data sparsity, influence cost~\cite{extensor}.
% \chris{The above sentence is confusing because I do not know the difference between a input and a hyper-parameter that sets layer shape.}
We consider efficient mapping space search for input-dependent mappings to be important future work.

%\chris{this next sentence seems out of place.  why are we talking about ASICs here?  I was expecting this sentence to just say how for accelerators today, the search is typically done at compile-time (precisely because the DL algorithms are data-oblivious -- for the most part.}
%However, typical hardware accelerator design process starts with a configurable cost model of the hardware.
%With such a model, one can perform such a search even during the design-time and choose to hardwire the optimal mapping into the hardware, turning it into an ASIC.
%Overall, the mapping space search is a crucial part in each phase of the design process of a specialized hardware.

% Interestingly, the mapping space search may need to be performed in design-, 
% For example, an ASIC might \chris{have?} with a fixed mapping~\cite{eyeriss,scnn,ucnn,cnvlutin} of the algorithm to accelerator needs to perform the mapping decisions in design-time.
% \chris{why is this called mapping space search and not hardware design space search?}
% Similarly, a flexible accelerator~\cite{maeri,dna,morph} that can support different mappings may perform the mapping in either compile- or run-time.
% In all the above cases, a search is necessary in $M$ to find an optimal mapping that minimizes the execution cost.

% \begin{verbatim}
% your
% code
% example
% \end{verbatim}



% The design space of an application specific hardware accelerator is a superset of all decisions that the architects need to make to design a functional hardware that runs the algorithm of interest.
% One can visualize this design space as a combination of architectural and algorithmic design space, as depicted in Figure~\ref{fig:design_space}.
% The mapping space $M$ is a subset of the design space that has a combination of both architectural and algorithmic design space.
% The design decisions from $M$ at least ensures the functional correctness in execution, further has the potential to impact the performance, efficiency, area, and other aspects of the accelerator.
% A subset of the mapping space $M$ is the flexible mapping space, where the design decisions are 
% The mapping space is not only a bridge between the 


% The other set of design decisions that are independent of the algorithm of interest form the architectural parameters $a$ and the set of all valid parameters form the architectural space $A$.
% However, the choice of $a$ has an impact on the efficiency of execution of algorithm on the hardware

% Every mapping $m \in M$ is a valid

\subsection{Cost Function}
\label{subsec:cost}
The cost function $f$ (Equation~\ref{eq:schedule}) estimates the cost of running the given mapping $m$ on the given hardware accelerator $a$.
This serves as the objective for optimization in the mapping space search.
It is up to the designer to formulate the cost function based on the design criteria.
For example, the cost function can be formulated as a weighted sum or product of several factors, or as a prioritized order of measurable metrics~\cite{timeloop}.
%\chris{is ``prioritized order of measureable metrics'' a common term?  Also, it doesn't sound like a scalar (which is what I need for f).}\kartik{Angshu/Po-An?}
For example, $f(a,m) = \sum_{k=0}^{K-1} w_k f_k(a, m)$
where $K$ is the set of all the factors considered by the designer and $w_k$ is the importance assigned to the $k$-th factor.
Factors can include various measures such as power, performance, or meta-statistics such as the number of buffer accesses, etc., and designers may choose to assign appropriate weights for each of the costs based on the requirements/factors.
For example, if $f_k$ represents the number of DRAM accesses, $w_k$ might represent the energy per DRAM access.
Importantly, the function computing each factor $f_k$ need not be smooth, differentiable, etc.
%\angshu{Timeloop uses a user-specified lexicographic (i.e., prioritized) order of measurable metrics. For example, you can search for optimal perf, but if you have 2 mappings with the same perf, you can select based on energy.}
%\chris{can one think of this as a weighted sum?  E.g., if the $f_k$ for perf is equal across 2 mappings, then they cancel and we are left with the term for energy as you say.}
%\angshu{No. With a weighted sum I may, for example, be able to have so large an energy benefit that it overrides a performance deficit *Unless* I know a-priori what the maximum possible energy is, in which case I can scale the performance weights by that amount --- sort of like creating a multi-digit number space, or flattening a multi-dimensional space. You need to know the maximal bounds of each dimension to flatten it. A lexicographic ordering achieves the prioritization naturally. Hope I'm making sense. If not I can explain with an example.}
%For reference, we provide an example mapping space in Section~\ref{subsec:mapspace_example}.


\section{Example Mapping Space: 1D-Conv}
\label{subsec:mapspace_example}

\newcommand{\inp}{\mathsf{I}}
\newcommand{\out}{\mathsf{O}}
\newcommand{\filt}{\mathsf{F}}

We now describe the mapping space for a hardware accelerator designed to perform 1D-Convolution (1D-Conv) with energy-delay product as the cost function.
This represents a simplified version of the accelerator and algorithm (Convolutional Neural Nets/CNNs) that we evaluate in Section~\ref{sec:eval}, and we will refer to the example in Section~\ref{sec:method} to explain ideas.

Algorithmically, for filter $\filt$, input $\inp$, and output $\out$, 1D-Conv is given as
\begin{align}
&\out[x] = 
    \sum_{r=0}^{R-1} 
        \inp[x+r] * \filt[r] \label{eqn:1dconv} \\
    \nonumber &0 \le x < W-R+1
\end{align}
for input width $W$ and filter size $R$.
Using the terminology in Section~\ref{subsec:mapspace_search}, the 1D-Conv algorithm forms a family of problems, where each problem $p$ corresponds to a specific setting of $W$ and $R$.
% leading to a mapping space $M$ for each problem, or setting of $W$ and $R$.

1D-Conv in Equation~\ref{eqn:1dconv} can be represented as a loop nest:
\begin{lstlisting}[language=C,caption={\small Untiled 1D-Convolution.},captionpos=b,label={code:untiled}]
for(x=0; x<W-R+1; x++) {
	for(r=0; r<R; r++) {
		O[x] += I[x+r] * F[r]; } }
\end{lstlisting}
We represent the ordering of the loops in the above loop nest as $W\rightarrow R$, meaning iteration over $W$ and $R$ is the outer and inner loop, respectively.
%\chris{The loop order notation is still not fixed!}
Note that due to the commutativity of addition~(ignoring floating point errors), we can freely interchange the loops, i.e., as $R\rightarrow W$.
% \chris{problems with previous sentence: 1) we don't say arithmetic is fixed point so commutativity might not even hold.  2) it doesn't seem relevant at this point because we just defined the loop nest, not the map space.}

We can also add additional levels to the loop to model tiling or blocking.
For example, if $\filt$ cannot fit in a buffer, we can tile it as shown here:
%\chris{please someone sanity check my code}
\begin{lstlisting}[language=C,caption={\small Tiled 1D-Convolution.},captionpos=b,label={code:tiled}]
for(rc=0; rc<Rc; rc++) { // Rc=ceil(R/Rt);
  for(x=0; x<W-R+1; x++) {
    for(rt=0; rt<Rt; rt++) {
      roff = rc*Rt + rt;
      O[x] += I[x+roff] * F[roff]; } } }
\end{lstlisting}
%\chris{when you change the pesudocode style, make sure the symbols in text use the same font as the pseudocode}\kartik{Hard to match}
That is, we complete the 1D-Conv for an $R_t$ chunk of $\filt$ at a time, adding an outer loop over the number of tiles $R_c$.
This loop nest is therefore written as $R_c\rightarrow W\rightarrow R_t$. 
Beyond tiling, we can describe parallelism in the computation by conceptually pre-pending \texttt{parallel} before a given loop(s), indicating that iterations of that loop can run in parallel.

\begin{figure}[t]
\begin{centering}
  \includegraphics[width=0.70\columnwidth]{figures/accelerator.pdf}
  \caption{A basic hardware accelerator with $M$ processing elements, on-chip buffer with $N$ banks, and a NoC.}
  \label{fig:accelerator}
\end{centering}
\end{figure}

An example target accelerator for the 1D-Conv algorithm is depicted in Figure~\ref{fig:accelerator}.
At a high-level, it has $M$ processing elements, an on-chip buffer with $N$ banks allocatable to different tensors at bank granularity, a flexible NoC that can be optimized for different communication patterns such as broadcast, unicast, etc.

Let us assume that the accelerator's programmable attributes are:
\begin{enumerate}
    \item $P_0 = \mathbb{R}^3$: a 3-tuple indicating the percentage of banks allocated to each of $\inp$, $\out$, and $\filt$.
    \item $P_1 = \mathbb{Z}^{3}+$: a 3-tuple representing the tile shape of $\inp$, $\out$, and $\filt$ to be fetched from DRAM.\footnote{Note that in 1D-Conv, tiles are 1-dimensional.  Hence, shape is representable as a scalar.}  The $+$ is to facilitate multiple levels of tiling, if applicable.
    \item $P_2 = \{W\rightarrow R, R\rightarrow W\}$: loop order for the untiled 1D-Conv algorithm represented in Code~\ref{code:untiled}. 
    To support more loops levels due to tiling (as in Code~\ref{code:tiled}), we add additional tiled loop orders to $P_2$ (e.g., $R_c\rightarrow W\rightarrow R_t$).
    %Programmable accelerators with tiling support require as many loop orders as the levels of tiling, as represented in Code~\ref{code:tiled}, which we represent with $+$ for simplicity.
    %\chris{why do we need + if each element is a complete loop order?}\kartik{+ is more loop orders are needed with additional tiling levels}
    %\chris{also: it is confusing that you say "untiled" in the first sentence, and then talk about tiling in the second sentence}\kartik{Why? Distinguishing the two. Any better way to write this? Ignore the tiled version?}
    %\chris{this is really quite confusing.  For a given level, the only thing $P_2$ encodes is which tensor is being iterated over at that level.  But I need to know other information, e.g., stride.  I think you are implicitly assuming the forms take a specific form, but that needs to be stated explicitly.}\kartik{Changed how the loop order is defined, I think this makes more sense and is consistent with earlier note about loop order.}
    
    \item $P_3 = \mathbb{Z}+$: the loop bound for each loop, e.g., $R_c, W+R-1, R_t$ in Code~\ref{code:tiled}.
    Note, we write this attribute explicitly for clarity.  In this example, loop bound can be inferred from the current assignment to $P_1$ and $P_2$. 
    \item $P_4 =  \{\mathrm{unicast},\;\mathrm{multicast},\mathrm{broadcast}\}^3$: NoC communicating patterns for each of the 3 tensors.
    \item$P_5 = \mathbb{Z}+$: Amount of parallelism per PE for each loop level.
\end{enumerate}
% \chris{kartik: check changes I made to P1, P2, P3}

\textbf{Mapping Space.} 
Given the above, one can construct a mapping space $M_{a,p}$ for the accelerator and specific 1D-Conv problem (i.e., the specific setting of $W$ and $R$).
The accelerator has $D=6$ programmable attributes and the mapping space size is bounded by the size of the Cartesian product of assignments to each programmable attribute.
As discussed in Section~\ref{subsec:mapspace_search}, the mapping space size will be smaller than this upper bound, as some complete assignments to programmable attributes are invalid, e.g., $R_t < R$ must hold since $R_t$ is a tile of $R$. 

\textbf{Cost Function.} In the above example, the cost of a mapping $f(m)$ is defined as $\mathrm{energy}*\mathrm{delay}$.
This can be obtained by simulators or analytical models that represent the actual hardware or using the actual hardware itself.
For example, Timeloop~\cite{timeloop} (which we use in our evaluation) is a tool that can calculate mapping cost for algorithms representable as affine loop nests (e.g., convolutions).
%on a given programmable accelerator targeting any algorithm that can be represented with an affine loop nest~(e.g., convolution) using an analytic model that performs bottleneck analysis on each hardware component. 
% Different choice of the programmable attribute of the accelerator may affect the cost differently
% $\mathrm{energy}$ may be the dot product between the number of accesses to each buffer, e.g., the banks and DRAM, and the cost per buffer access in Joules.
% $\mathrm{delay}$ may be calculated using simulation or an analytic model.


\subsection{Challenges in Mapping Space Search} % and Constructing Gradients}
\label{subsec:challenges}

\begin{figure}[h]
\begin{centering}
  \includegraphics[width=0.95\columnwidth]{figures/erro_surface.png}
  \caption{Cost surface plot for the accelerator we evaluate in Section~\ref{sec:eval} for CNNs. Darker red indicates higher EDP, and darker blue indicates lower EDP. Mind Mappings approximates this non-smooth surface with a differentiable surrogate to enable gradient-based optimization.
  }
  \label{fig:error_surface}
\end{centering}
\end{figure}

A major challenge in mapping space search is the nature of cost function $f$, which is non-convex and non-smooth.
For example, consider the 1D-Conv example from the previous sub-section.
The cost of a mapping $f(m)$ is influenced by the various programmable attributes $P_d$ in subtle ways.
For example, consider $P_0$, the attribute that represents buffer allocation for each operand/result tensor $\inp$, $\out$, and $\filt$.
If the $\filt$ tensor is 1~KB in size and allocation falls short of 1~KB, the mapping cost will see a significant energy bump as valid mappings will be forced to tile $\filt$, requiring some operand(s) to be re-fetched multiple times to fully compute $\out$.
%meaning will need to be refetched to calculate every element of $\out$.
In other words, seemingly minor changes to mapping $m$ can result in non-smooth changes to the overall cost $f(m)$.
%\chris{equating irregular to non-smooth is a bit sketchy.  I don't understand why we can't simply say that Timeloop is not differentiable.}\kartik{Get rid of irregular term?}\chris{well, I think irregular is more accurate, no?  It is informal and I don't see a correct formal statement to make here (yes, it is non-smooth, but is.}

%would dramatically change the data access pattern, which will significantly influence statistics such as energy.
To illustrate this, Figure~\ref{fig:error_surface} plots the cost surface
for the programmable accelerator running Convolutional Neural Network (CNN) layers that we evaluate in Section~\ref{sec:eval}.
In the figure, the $x$- and $y$-axis represent different choices of tile sizes for two different input tensors, 
while the $z$-axis represents the cost $f$ in terms of the energy-delay product (EDP).
Evident from the plot, the search space is spiky and non-smooth in nature.
Due to this, obtaining useful statistics such as the gradients~(first-order), Hessians~(second-order) of the search space is not possible, requiring the search for optimal mapping~(Equation~\ref{eq:schedule}) to use black-box optimization approaches such as Simulated Annealing~\cite{simanneal}, Genetic Algorithms~\cite{genetic}, etc.
Making matters worse, the search space is clearly non-convex, i.e., many local minima, making the search even harder.
Given the humongous search space size~($\approx10^{25}$ in this example), black-box optimization approaches struggle to find high quality mappings in few iterations.

%\kartik{Please read now, does the Figure add value here? I think it at least shows the reader that the problem is not easy.}
%\chris{its better, but I think we should still say something about "many local minima" as that is what pops out at me before "non-smooth"}
%\kartik{Sure, I think it gels well with local minima subsection in S4. See the new sentence in last pargraph}
% \chris{
% I think there is a lot about Fig 2 that could confuse people.  We need to discuss.

% a) I really can't tell from looking at it if it is non-smooth or smooth.  The search space is discrete, in which case it is automatically non-smooth, no?  So why do I need a figure?

% b) Continuing from (a), the main thing I observe from Fig 2 is that there are many local minima, i.e., if I fix one dimension and dial up/down the other, the space isn't convex.  But having a diff. surrogate isn't going to help with that.

% c) I can't tell whether there are many or one global minima.  For MM to be effective, I think we want evidence of many global minima, right?  

% d) (IIRC this was Hughes' confusion) It isn't clear why the space has to look like this.  I.e., is your encoding of tile size just poor?  E.g., (as Hugh put it) why not just encode the domain of tile sizes so that cost is monotonically increasing.  That isn't practical because it depends on the input, but there isn't enough text right now to explain this.  We don't even say that the tile size programmable attribute is encoded as (presumably?) an integer.}
















%The cost function $f$ is generally  non-convex, non-differentiable and non-smooth in nature for hardware accelerators due to the abrupt variations in cost across different mappings.
%For example, as the size the data assigned to an on-chip buffer exceeds the size of the buffer, several execution characteristics such as power consumption may drastically change as one may need to tile the data to improve locality.
%\chris{one may need to change the algorithm from an untiled to tiled implementation}
%This makes the cost function highly non-smooth in nature.
%Additionally, frequent uses of \chris{non-linear} functions such as \emph{ceil}, \emph{abs}, etc., contributes to the non-differentiability of the cost function.
%\chris{unclear where these would come up}


%\chris{I think this/next sub-section can be improved.  1 - next sub-section needs to give more precise detail on what the mapping space is (see below comments -- saying ``1 param'' is too vague).  2 - sub-subsection should illustrate WHY the space is non-smooth.  E.g., show a situation where you might want to be output stationary, and then change the inputs and give some intuition for why you might want a different dataflow.  Depending on how its written, I could see you reversing the order of E and F as well: example fist, then explain why problem is hard.}

%\angshu{So the smoothness depends on how the set of mappings is enumerated into a multi-dimensional integer space. For example, the space of loop permutations can be mapped onto a space of integers called a "factoradic" space. Each integer in the factoradic space gives you a specific permutation. You can imagine how the cost across this factoradic space could have awful smoothness. But is there a better way to order the permutations to improve smoothness? Maybe, but I haven't thought too deeply about it. Makes me wonder if we should think of embeddings.}
%\chris{I am going to say in general, non-smooth to keep things simple.  thoughts: The issue of whether there exists an embedding s.t. the space is smooth is interesting.  On one hand, every graph is planar in 3 dimensions which suggests we can build smooth embeddings -- if the gradients were to take us precisely along edges of the graph from one point to another.  But in practice gradients aren't this good and we will hit other vertices on the way, which leads to non-smoothness.  One might be able to embed in higher dimensions to get around this, but that starts to defeat the purpose of the embedding.}
%%% marking this comment as resolved, although it is worth thinking about after deadline

% For example, a design that considers power and performance to be of equal importance can frame the cost as $0.5f_{power} + 0.5f_{perf}$.

% \subsection{Mapping Algorithm to Accelerator}
% As touched upon in Section~\ref{sec:intro}, once the architectural parameters are selected based on the budgetary constraints, the next step is to map the algorithm to accelerator.
% While the design decision of architectural parameters is a design-time decision, the mapping decision can be in design-, compile-, or run-time.
% \begin{itemize}
%     \item \textbf{Design-time:} In cases of ASICs, the algorithm mapping may be hardwired into the hardware, thus requiring an algorithm-accelerator mapping space search in design-time.
%     For example, several earlier works in deep learning accelerators hardware the mapping in the hardware~(also referred to as 'dataflow`)~\cite{eyeriss,scnn,ucnn,cnvlutin}.
%     \item \textbf{Compile-time:} A flexible accelerator could support varieties of mappings, hence a compiler might perform the mapping during compile-time based on the efficiency requirements.
%     We have seen several works recently that are flexible to different mapping strategies~\cite{maeri,dna,morph}. 
%     \item \textbf{Run-time:} A flexible accelerator that can support different mappings in run-time might perform the mapping search in run-time based on the current availability of compute and memory resources.
%     We predict that areas such as sparse tensor algebra can benefit from such run-time mappings, as utilization of resources can not be determined at compile-time.
% \end{itemize}

% Therefore, while the algorithm-accelerator mapping can happen at any stage in the design process, developing an effective and systematic approach to perform mapping space search remains crucial. 


==> method.tex <==
\section{Method}
\label{sec:method}

% \chris{S2 uses the term problem, S4 uses the term algorithm.  Need to decide which and be consistent.}

% \chris{I put "CHECK" next to text that is related to map space IDs.  In general, this is all very confusing as written.  1) We don't properly define "Parameterized instance" or describe hyper-params vs. inputs/provide an example.  2) The discussion uses many names to describe the same thing (parameterized instance, parameters, hyper-parameters, problem shape, ID).}

% \chris{I suggest moving appendix A back into the main body after S2.  We use it as an example in this section and if we move it back I think we could make further use of it (e.g., we briefly allude to different map spaces having different W R.  We can call this example out as soon as we mention "sample from multiple map spaces" the first time.)}

%\chris{SYNCH this with S2 terminology after the pass}
%\chris{Do a pass: make sure it is clear we build only 1 surrogate model for many shapes}
%\chris{algorithm to problem}

%\chris{CHRIS HAS LOCK}

%%%%%%%%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%%%% 

\begin{figure*}[t]
\begin{centering}
  \includegraphics[width=\textwidth]{figures/search_process_clubbed.pdf}
  \caption{Mind Mappings search procedure. \textbf{Phase 1:} Training the surrogate model $c^*=f^*(m, p_{id})$ based on (mapping, problem id, cost) tuples ($m$, $p_{id}$, $c$).  DNN (surrogate) weights $w$ are trained with back-propagation. \textbf{Phase 2:} Given a target problem $p_{target}$, use the trained surrogate model to iteratively guide a random initial mapping $m @ 0$~(``mapping at search iteration 0'') towards an optimal mapping $m_{opt}$. In each iteration, $m @ t$ is updated using back-propagation with a gradient $\nabla$ of $f^*$ based on $m @ t$ with a learning rate $\alpha$. The trained model weights $w$ and the target problem $p_{target}$ are held constant in this phase.
  %\chris{the notation for m0 ... mt is broken, because we use subscripts to index into the mapping vector already.  I suggest a new notation, e.g., $m\@0$ ... $m\@t$ to indicate the mapping as it evolves in phase 2.  I changed it in the caption and Phase 2 text.  Needs to be changed in figure.}
  %\chris{whatever notation we use, explain it in the caption}\kartik{CHECK}
}
  \label{fig:training}
\end{centering}
\end{figure*}

% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.5\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/method-phase1-cropped.pdf}
%     \caption{\label{fig:training:a}Phase 1: training the surrogate model $c^*=f^*(m, id)$ based on (mapping, map space id, cost) tuples ($m$, $id$, $c$).  DNN weights are trainable.}
% \end{subfigure}
% %
% \begin{subfigure}[t]{0.5\textwidth}
%     \centering
%     \includegraphics[width=.9\columnwidth]{figures/method-phase2-cropped.pdf}
%     \caption{\label{fig:training:b}Phase 2: Given a map space id $id_{target}$ and target cost $c_{target}$, which identifies a target map space: use the trained surrogate model to iteratively update a random initial mapping $m_0$ towards an optimal mapping $m_{opt}$. In each iteration, $m_{t}$ is updated using back-propogation with a gradient $\triangledown$ of the estimated loss with a learning rate $\alpha$.
%     The (initially random) mapping $m_t$ is trainable.}
% \end{subfigure}
% \caption{\label{fig:training} Proposed search method.}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%% \Figure %%%%%%%%%%%%%%%%%%%%%%%

%\chris{check consistency: mapping space search.  map space.}

%\chris{inconsistency: previously, we call it "map space search".  Here it is called "mapping space search".}\kartik{God catch, Fixed} \chris{still seems to be a problem}\kartik{Map space search --> Mapping Space Search, but map space itself is retained. I can't see any other map space search occurences.}

Due to the non-smooth nature of the cost function described in the previous sections, designers are forced to use black-box optimization approaches to find optimal mappings.
By definition of being black box, they cannot take advantage of structure within the accelerator cost function, which puts them at a disadvantage in effective mapping space search.
Mind Mappings circumvents this by \emph{approximating} the search space as a smooth, differentiable function.
This turns mapping space search into a white-box optimization problem, and enables gradient generation to improve the search.

Mind Mappings is a two-phase procedure, as shown in Figure~\ref{fig:training}.
We start with a target algorithm.
The goal is to find low-cost mappings for a potentially unbounded number of target problems given that algorithm.
To accomplish this:
First (Phase 1, Section~\ref{subsec:func_approx}), we train a \emph{differentiable} surrogate model to approximate the accelerator's cost function for all problems making up the target algorithm.
%
Second (Phase 2, Section~\ref{sec:design:mapping_search}), we perform Gradient Descent on the surrogate model to generate low-cost mappings for the target problems. 
Phase 1 and 2 are performed offline and online, respectively.

% Phase 1 can be expensive.
% To amortize/reduce its cost, the goal is to train the surrogate to generalize to unseen problems and to reuse the surrogate 
% across the potentially many problems in Phase 2.
% For example, given 1D-Conv from Section~\ref{subsec:mapspace_example}, Phase 1 trains the surrogate on mappings corresponding to representative $W$ and $R$ values, so that the surrogate will later be able to interpolate and return accurate costs for mappings belonging to \emph{unseen} $W$ and $R$ values.
% Then, Phase 2 uses the surrogate to search for low-cost mappings for those unseen $W$ and $R$ values.
% That is, the cost to train the surrogate is amortized because it is trained once, offline per target algorithm.

To amortize surrogate training cost (Phase 1), 
we train the surrogate to generalize to unseen problems and 
reuse the surrogate across the potentially many target problems in Phase 2.
For example, given 1D-Conv from Section~\ref{subsec:mapspace_example}, Phase 1 trains the surrogate on mappings corresponding to representative $W$ and $R$ values, so that the surrogate will later be able to interpolate and return accurate costs for mappings belonging to \emph{unseen} $W$ and $R$ values.
Then, Phase 2 uses the surrogate to search for low-cost mappings for those unseen $W$ and $R$ values.
That is, the surrogate is trained once, offline per target algorithm.

%, which is an online procedure.

% For example, {W,R} values set for the 1-D Conv example in Section~\ref{sec:background:example}.

%That is, to apply Mind Mappings we start with a target algorithm.
%The goal is to find a low-cost mapping given a target problem $p$ (which induces $M_{a,p}$) for that algorithm.

%\chris{there should be a note about functional correctness here.  I.e., I have no idea what the valid mappings for an unseen W/R will be relative to the overall map space for that W/R.  We need to do a functional correctness check at the end.}\kartik{Not sure if we should complicate about validity here}
%\chris{we need to be more explicit about how often we expect the surrogate to need to be trained.  I.e., if you have an algorithm with parameters X, you should not expect the surrogate to generalize to an algorithm with parameters Y.  It's a bit more subtle, since even if your target algorithm does have parameters X, that still doesn't mean the surrogate will generalize (since which mappings in each map space are valid need not be the same even given two map spaces with the same parameters).}

We now discuss Phase 1 and 2 in more detail.
We rely on the 1D-Conv example from Section~\ref{subsec:mapspace_example} to explain ideas.

%Figure~\ref{fig:training} gives an overview of both phases.
%In this section, we elaborate on both the steps of the search procedure and describe additional challenges faced during the procedure.
% \angshu{Are you making an explicit distinction between "algorithm", "problem" and "problem instance"? All 3 terms are used here. I think we need a quick definition in parenthesis, e.g., "Problem instance" is a parameterized instance of an "algorithm".}

\subsection{Phase 1: Approximating the Map Search Space}
\label{subsec:func_approx}

%\chris{say somewhere that f* takes m and pid as input}\kartik{Check the red text}

As discussed in Section~\ref{subsec:map_space}, the cost function $f$ that maps input mappings to a designer-defined cost is non-smooth and non-differentiable.
To make $f$ differentiable, which will allow us to generate gradients, we use \emph{function approximation}~(FA) with differentiable surrogates.
FAs are often used to reduce a function's dimensionality, which has been shown to simplify optimization problems in different fields such as reinforcement learning~\cite{func_approx_0,func_approx_1}.
It has also been used in prior works~\cite{surrogate_0,surrogate_1, ithemal, tvm} to improve the speed of evaluation of $f$ to enable rapid searches.
%\angshu{What is "state space"? It hasn't been defined before.}

With FA, we generate a smooth, differentiable approximation of the cost function, denoted \fapprox, called the \emph{surrogate}.
Given a mapping $m$ and problem $p$, the surrogate predicts the cost $c^* =$ \fapprox$(m,p)$, where $c^*$ approximates the actual cost, $c=f(m)$. Therefore, each surrogate is specialized for a given accelerator and the target algorithm, but should be able to return accurate costs for the different problems making up the algorithm.
%by training a surrogate model to approximate the cost function as a smooth, differentiable function.
Notice, $p$ is specified as an input to \fapprox.
This is a notational convenience that will be important in Phase 2.

While there are multiple choices of differentiable surrogate functions, we use Multi-layer Perceptron~(MLP)-based Deep Neural Networks~(DNNs) in this paper as 
they are known to be capable of modeling high-dimensional functions 
and feature a mature training infrastructure due to the recent advances in Deep Learning.
We leave the question of whether simpler, differentiable models are sufficient as future work.
%since they not only capture the non-linearity of the cost function effectively, 
%but also enable us to utilize 
%due to the recent advances in training DNNs from the machine learning community. 
%\angshu{How do we know that it captures the non-linearity of the cost function effectively? Is this a hypothesis or prior work?}

Figure~\ref{fig:training}, Phase 1, gives an overview of how to construct/train the surrogate. %the procedure to train a surrogate model to approximate the cost function of the accelerator as a smooth, differentiable function.
At a high level:
We construct a training dataset of input mappings $m$ and their associated costs $c=f(m)$, where
% \chris{why not just say c = f(m) then?}
%by uniformly sampling from the family of problems for the target algorithm-accelerator pair.
%For example, uniformly sampling from different choices of $W,R$ in 1D-Conv and then uniformly sampling from the map spaces given by those values of $W,R$. %, $M_{a,p}$.
%\chris{may want to use other notation, e.g., $M_{a,(W,R)}$.}
$f$ is the accelerator's reference cost model.
Each element in the training set is stored as a 3-tuple: mapping $m$, problem identifier $p_{id}$ (from which $m$ was sampled) and reference model cost $c$.
%Each mapping is stored in the training set alongside an 
%To differentiate mappings belonging to different map spaces (problems), which will be important in Phase 2, each mapping $m$ is labeled with an identifier indicating its problem.
%For example, the identifier for 1D-Conv can be a tuple stating the concrete assignment to $W$ and $R$.
%Then, each mapping is labeled with its actual cost $c$ (using the accelerator's reference cost model).

%A sampling is performed from the map space to generate valid mapping vectors $m$ which is then passed as an input to a deep neural network~(DNN).
%The mapping vector $m$ is also used to generate the actual cost using a reference model of the hardware accelerator.
The distance between the predicted cost, \capprox, and the actual cost $c$ is used to generate a loss, which is used to train the surrogate using back-propagation~\cite{backprop}.
The training procedure can be carried out until satisfactory loss is reached, and well-studied techniques in deep learning can be used to improve the speed of convergence~\cite{dropout, Imagenet}.

Superficially, the above process is a ``standard'' supervised training with Stochastic Gradient Descent~(SGD), widely used in modern deep learning approaches.
Getting it to work properly for mapping space search, however, entails addressing multiple issues, as described below.

\subsubsection{Generating the Surrogate Model Training Set}
\label{sec:method:gen_train}

The first step is to build a training set to train the surrogate model.
We face the following questions:

% \begin{enumerate}
%     \item What mappings should populate the training set? \label{step:1}
%     \item How to sample a mapping from each map space? \label{step:2}
%     \item How to associate a mapping with its map space? \label{step:3}
%     \item How to calculate cost for each mapping? \label{step:4}
% \end{enumerate}

\textbf{(1) Which map spaces should be used to populate the training set?}
The naive approach is to populate the training set with mappings associated with a single problem for the target algorithm.
% The naive approach is to populate the training set with mappings from a single map space associated with the target problem $p$.
%\chris{I don't like saying "target problem p" because it gives the impression Phase 2 will only be run for one target problem.  I have been saying: start with a target algorithm.  We will have potentially many target problems.}
%\chris{above doesn't make sense.  what is the target problem p?  do you mean algorithm?  we don't have a target problem until phase 2.} \kartik{We have defined what a problem is in Section 2. We do need problem in phase 1, each mapsapce is associated with a problem}
This approach fails because the resulting surrogate will not generalize to unseen problems, requiring us to re-train the surrogate for each new problem we encounter.
%\chris{... for different parameterizations of the same algorithm?}\kartik{Problems already mean parameterization of the algorithm}
For example, a new surrogate will be needed every time the $W,R$ settings change for 1D-Conv---clearly undesirable.
Instead, we generate training points by uniformly sampling from multiple map spaces, thereby generalizing the surrogate across the family of problems associated with the target algorithm.
We empirically observe that the model is able to interpolate and predict correctly for problem instances it hasn't seen before.
% Note that this is similar to the state-of-the-art supervised learning approaches--better the dataset, higher is the generalization.
% \chris{this last sentence isn't needed}

% Selecting representative map spaces at training time is important, as our goal in Phase 2 is to search for mappings that belong to map spaces \emph{not seen at training time}, i.e., that belong to unseen $W$, $R$ settings.

\textbf{(2) Based on the choice of map spaces, which mappings should we sample to populate the training set?}
There are three issues here. First, we must be able to check if a mapping is valid, i.e., belongs to a specific map space.
For this, we assume there exists a membership testing function $\mathsf{isMember}(m,p)$ for every accelerator $a$ which returns true if $m\in M_{a,p}$ and false otherwise.
%\chris{shouldn't isMember also have 'a' as an input?}\kartik{Assumed isMember is defined for the accelerator by the cost function}

Second, we must decide whether to populate the training set with only valid members of each map space---i.e., mappings that are functionally correct for their given problem---or also consider invalid mappings.
In this work, we only populate the training set with valid mappings.
Considering invalid mappings may enable the surrogate 
%\chris{this is a bit unclear because you are referring to phase 2.}\kartik{Readers have some familiarity that the surrogate will be used for the search later}
to better avoid functionally incorrect mappings in Phase 2, e.g., by assigning them infinite cost.
However, this may face implementation challenges such as exploding gradients and slow convergence~\cite{exploding_grad}.
% We consider exploring this future work.

Third, we need to decide on a sampling strategy to sample from each map space.
One option, which we use in this work, is to sample uniformly at random. 
Specifically, given a problem $p$, we sample from the associated map space $M_{a,p}$ uniformly to generate a mapping and re-sample if the mapping is not valid (see above).
This ensures a reasonable representation of the map space, but might suffer from under-sampling from regions that are more important from a training perspective.
Other advanced sampling methods can be used, such as sampling from a probability distribution trained to maximize the amount of learning per sample~\cite{gumbel}.
As seen from our evaluation~(Section \ref{sec:eval}), uniform random sampling facilitates training well and therefore we leave improved sampling methods to future work.
%\chris{do we need this last sentence?}\kartik{I think it adds some value, I don't have a strong preference}
%We found consider improved sampling methods to better explore the space as an important future work.

\textbf{(3) How to uniquely associate each mapping $m$ with its map space $M_{a,p}?$}
It is possible to have the same mapping $m$ present in multiple map spaces, where each mapping instance has a different cost $c$.
Therefore, to ensure correct generalization of the surrogate across different problems for the given algorithm,
we must uniquely identify each mapping in the training set with its map space.
For this, we need to tag each mapping $m$, added to the training set, with a problem identifier $p_{id}$, unique to the map space associated with its problem $p$.
%\chris{huh? this sounds like there are multiple map spaces associated to a given problem.}\kartik{rephrased}
In this paper, we encode each $p_{id}$ as the specific parameterization of the problem, e.g., a tuple indicating the $W,R$ values associated with the problem for the 1D-Conv algorithm~(Section~\ref{subsec:mapspace_example}).
%\chris{when will the above ever happen?  isn't the real reason we need pid just because of Phase 2?}

\textbf{(4) How to calculate cost per mapping?}
To train the surrogate, we require a reference cost $c=f(m)$ that can be used to calculate the loss w.r.t. surrogate's predicted cost \capprox. %, to calculate the loss for training the surrogate using standard supervised training techniques.
% \chris{"gradients for back-propagation" is a bit confusing because you mean for Phase 1, but we have reserved the word "gradients" for Phase 2.  Suggestion: "to calculate the loss for training the surrogate".}
This can be estimated via running the problem with mapping $m$ on the target hardware or using a cost function estimator such as those described in Section~\ref{subsec:cost}.
As this is a one-time, offline procedure that generalizes over different problems for the target algorithm, its cost is amortized over multiple mapping space searches performed using this surrogate.
% In this paper, we use Timeloop~\cite{timeloop} to generate costs.
% Costs are generated during training set creation time and stored with each mapping during training.

We now describe input mapping vector and output cost representation.
We describe ideas and challenges here.
The concrete representations we use for our evaluation are detailed in Section~\ref{subsec:eval:sensitivity}.

\subsubsection{Input Mapping Representation}
\label{sec:method:input_rep}

%\\ 
As described in Section~\ref{subsec:mapspace_search}, the mapping vector $m$ is a $D$-tuple consisting of the accelerator's programmable attributes, which needs to be converted to a representation that can be used to train the surrogate.
There are two issues here.
First, while each programmable attribute $P_d$ can have different representations, e.g., vector, integer, float, boolean, etc., the input to the surrogate needs to be a single vector of floats.
We resolve this by converting each attribute to a scalar or a vector of floats, flattening multiple vectors into a final mapping vector as needed.
%\chris{why reals, not just floats?  it has to be floats, right?  FP is just a discretization of the reals, since reals require infinite bits to encode.  I surrounding later uses of "real" in slash chris so we can do something with them when we decide.}
For example, $P_4$ in 1D-Conv (Section~\ref{subsec:mapspace_example}) has 3 discrete choices, which can be converted to a vector of 3 floats which are one-hot encoded.
The choice of float for the mapping vector datatype isn't fundamental; in what follows, we refer to each float/element in the mapping vector as a value.

%\chris{is there an intelligent decision to be made here? it sounds like all encodings are equally good/bad.}\kartik{This is a hard question, because there are trade-offs with any encoding. I used trial and error make a choice on the encoding.}\chris{so you use one hot, or something else?  which others did you try?}\kartik{In case of loop order, explicitly stating the location in the order helped, i.e., if W-->R then 0 1, otherwise 1 0, where each bit indicates where the dimension is in the order.}\chris{I think these details are important and interesting.  Can you please elaborate what encoding you use for each prog. attribute?}

% In such cases, we add Gaussian noise to induce some smoothness before using them as an input.
Second, in some cases, it may be desirable to have variable-length mapping vectors for different problems~(e.g., to encode variable levels of tiling), but the input vector to the surrogate is often fixed~(e.g., as in a Multi-layer Perceptron).
%\chris{I am confused.  We never change the number of programmable attributes $D$.  We might change the number of reals needed to represent each attribute.  I assume that is what you mean?}
%\kartik{We don't in this paper as mentioned, but an accelerator could: support variable number of tiling/loop orders}.
While we deal with fixed-dimensionality mappings in this work, the above can be easily handled via embeddings~\cite{embedding}, a widely used method to deal with different input lengths in areas such as Natural Language Processing and Recommendation Systems.

Finally, we normalize each value in each mapping to have mean 0, standard deviation 1---in a process akin to input whitening~\cite{Alexnet, Imagenet}. 
That is, let $m'^{i}_{d}$ be the $d$-th value in the $i$-th mapping in the training set, where $m'$ means the mapping $m$ has been flattened into a vector of $D'$ values as described above.
Then, we normalize each $m'^{i}_{d}$ with respect to other $m'^{j}_{d}$ in the dataset.

%to have mean 0 and standard deviation 1, with respect to corresponding $m_d$ in other mappings $m$ in the training set.
%\chris{the above is confusing.  It isn't clear whether the $i$ in $m_i$ is to a specific attribute in $m$ or whether it refers to one of the many $m$ in the training set.  Suggest: notation $m^j_i$ to distinguish the two.}
%\kartik{I think we should simply say that we normalize the dataset to have a mean 0 and std 1, which is a standard practice[cite]}.

% Each attribute may itself be a complex datatype, e.g., a vector.
%Many of these attributes have discrete choices, e.g., loop order or NoC communication pattern.
% While there are advanced approaches to encode discrete-valued inputs, e.g., , we have found standard input normalization~\cite{efficient_backprop} to be effective, and use it in our evaluation.

% Specifically, we encode each attribute as a scalar or a vector of real value(s).
% For example, $P_0$ through $P_5$ in Section~\ref{sec:background:example}. 
% Attributes with discrete choices such as loop order or NoC communication pattern are enumerated and mapped to integer domains.
% %Non-numeric attributes, e.g., NoC communication, are mapped to integer domains.
% Some attributes become multiple reals, e.g., $P_0$ in the example becomes three reals.
% Next, we concatenate all attributes to form a vector of $d'$ reals, i.e., $m\in\mathbb{R}^{d'}$.



%While continuous parameters are easy to deal with in DNNs, discrete parameters pose a challenge.
%We use approaches widely used in areas such as Natural Language Processing~(NLP) that use an embedding layer~\cite{embedding} to convert discrete choices to a set of weights that are learnt during the training procedure of the main model.
%\chris{needs an example/possibly a figure}
%In these cases, we add Gaussian noise to induce some smoothness before using them as an input to the embedding layer. 

% Representation of the algorithm is in terms of relations between the data-types, loop bounds, etc., inspired by the representation in polyhedral models.
% The hardware description is in terms of the architectural template and properties, similar to the likes of \cite{timeloop}.
% The framework gives an interface where the search implementation can query for a random valid mapping for the training procedure.

\subsubsection{Output Cost Representation}
\label{sec:method:output_rep}

%\chris{wasn't clear if I should read this yet, so I haven't}\kartik{Unlocked}

A crucial decision to make is to choose a representation for the cost vectors $c$ and $c*$ that facilitates a high quality surrogate.
A straightforward approach, often used by prior works, is to represent costs as a combined statistic or the final target, such as EDP, performance/watt, etc.

Instead, we encode costs as a vector of \emph{meta-statistics} as we observed that this results in higher quality surrogates.
For example, for the surrogate we evaluate in Section~\ref{sec:eval}, we represent cost as a vector containing the energy spent accessing each level of the memory hierarchy by each data type (e.g., input/output tensor in 1D-Conv), compute utilization, total cycles, and total energy, although the final metric of interest is EDP.
We empirically found that this rich output representation enabled the surrogate model to achieve a $32.8\times$ lower mean-square error to the ground truth EDP, relative to surrogates that output EDP directly.

Additionally, we normalize the output cost vector with respect to a theoretical lower bound cost for the target problem, to reduce the variance in output values.
We use a conservative lower bound that assumes perfect data reuse and perfect compute utilization.
For example, for 1D-Conv from Section~\ref{subsec:mapspace_example}, the lower bound for cycles is given by $((W-R+1)*R)/max\_flops$ (assuming 1 cycle/FLOP), whereas the lower bound for energy is given by 
$(W + W-R+1 + R)$ times the energy needed to access each word of data once.
We evaluate an architecture with an inclusive buffer hierarchy, meaning that the energy needed to access each word once the sum of the energies per access for each level of the memory hierarchy.
%$\sum_{h=0}^{H-1} (W + W-R+1 + R) * cost\_to\_access\_level[h]$, where $H$ is the number of levels in the memory hierarchy
%\chris{you mean levels in the memory hierarchy?}
%$cost\_to\_access$ represents the energy to access one word for every hierarchy.
%\chris{for every level in the hierarchy?}
%\chris{I don't understand $cost\_to\_access[h]$.  Wouldn't the lower bound be "for every MACC, read L0" (as opposed to "for every MACC, read every level")?  The notation where $cost\_to\_access$ is accessed with the loop index is also confusing.} \kartik{What is a better way to write, all I am trying to communicate is that assume a data is read only once(perfect reuse), multiply with energy access}
We note that while this lower bound is possibly not achievable, it is only meant to give us a good normalization metric.

Finally, similar to inputs~(Section~\ref{sec:method:input_rep}), each value in the output vector is normalized to have mean 0 and standard deviation of 1 with respect to the corresponding values in other cost vectors in the training set.

% However, we empirically observed that this results in poor learning and search performance.
% We hypothesize the reason is that such combined statistics make the cost function $c=f(m)$ \emph{many-to-one}.
% For example, we might have different mappings $m1$ and $m2$ that map to the same $c$, e.g., total energy.
% This complicates training: the surrogate learns that some combinations of attributes result in same energy but not the direct relationship between attributes and cost, all else being equal.
% \chris{As I re-read this, I have the same confusion as always: If the gradients back-propagated through each meta-stat are the same, regardless of whether you present them to the loss function directly or hide them behind the aggregate statistic, why should there be a difference?}

% This in turn hampers the search quality by generating gradients only based on the combined statistics.

%While we want to judge mappings by combined statistics in Phase 2, w
% We have experimentally found that such representations for $c$ in Phase 1 result in low-quality surrogates during Phase 2.
% Our hypothesis is that combined statistics create ambiguity during training.
% For example, in Section~\ref{sec:background:example} we might have different mappings $m1$ and $m2$ that map to the same $c$, e.g., total energy.
% This complicates training: the surrogate learns that some combinations of attributes result in same energy but not the direct relationship between attributes and cost, all else equal.
%Yet, if $m1$ has more/less DRAM/buffer accesses than $m2$, generating gradients just based on total energy $c$ isn't sufficient information to teach the surrogate the relative cost of accessing DRAM vs. buffers.

% To address this issue, we 
% For example, counting the number of buffer accesses is a good proxy for energy efficiency, whereas compute utilization is a good proxy for performance.
% Meta-statistics make the mapping to cost relationship more one-to-one (which addresses the problem above), and (experimentally) significantly improve training and search quality.
% \chris{where is this in S5?  I would like to go over the methodology you used.}

% \chris{At what iteration / time point in training was this result obtained?  After training converges? (If so, not clear why we need a separate graph as the revision document says.)}
% \kartik{Yes, this is after converged training}
%We choose each statistic to be a proxy for final cost, e.g., reducing the number of DRAM accesses will help reduce total energy, so that back-propagating gradients in Phase 2 can be used to improve cost (Section~\ref{sec:design:mapping_search}).

% \subsubsection{Summary}
% To summarize (also see Figure~\ref{fig:training}):
% \begin{itemize}
%     \item Section~\ref{sec:method:gen_train}: We construct a training set of (mapping, map space ID, true cost) tuples, sampling only valid mappings from a set of representative map spaces.
%     The map space IDs require expert knowledge to encode.
%     \item Section~\ref{sec:method:input_rep}: Input mapping representation is a vector of reals, normalized (whitened) with respect to other mappings in the training set.
%     \item Section~\ref{sec:method:output_rep}: Output cost $c$ and \capprox is represented as a vector of meta-statistics.
% \end{itemize}

\subsection{Phase 2: Gradient Search to Find High-Quality Mappings}
\label{sec:design:mapping_search}

Phase 2, the online part of the search procedure, finds a low-cost mapping $m_{opt}$ for the target problem $p_{target}$, as depicted in Figure~\ref{fig:training}.
% \chris{Same issue as above.  Phase 2 takes as input a target problem.  But there is only one map space associated with it, not many.  When you write "unseen map spaces associated with p" it sounds like you mean p to represent the algorithm.}\kartik{Agree, fixed}
% For a given problem $p$,
% the search needs to find a mapping $m_{opt}$ that minimizes the cost function $f(m)$~(Equation~\ref{eq:schedule}). 
We achieve this by leveraging the differentiability of the surrogate model \fapprox~(Phase 1) 
% that represents an approximated version of the actual cost function $f$
to obtain gradients, where gradients represent the change in $m$ that maximally reduces the cost $f(m)$.
% \chris{I am confused.  We should be talking about minimizing cost for target problem in this opening paragraph, no?  Why are we talking about ctarget?  I see in the submission version we also talked about ctarget.  I think it is ok to briefly mention that the generalization of phase 2 is to minimize distance between cost of unseen mapping and ctarget, but we have to very quickly say that in our application, we also set ctarget equal to minimal cost.}
% \kartik{Yes, changed the text to not talk about c tragtet in the intro paragraph.}
With access to gradients, unlike black-box optimization approaches, we can perform powerful first-order optimization methods which, in effect, incrementally guide any random valid mapping $m$ towards $m_{opt}$ using Gradient Descent.
The key insight here is that, while the cost function representing the accelerator itself is non-differentiable, its differentiable approximation \fapprox \ should give us access to approximate gradients that can guide the search along the direction of steepest descent.
% Figure~\ref{fig:motivation} depicts this on a toy example.

% \chris{this example feels way out of place and is not helping me understand this section better.  I suggest removing it.}

% \begin{figure}[h]
% \begin{centering}
%   \includegraphics[width=0.75\columnwidth]{ASPLOS CR/figures/motivation.png}
%   \caption{\small Comparing Mind Mappings approach with approximate gradients generated from \fapprox with Gradient Descent using true gradients, as well Simulated Annealing, a popular black-box approach.
%   We optimize $f(x) = \sum_{i=0}^{N-1} x_i^2$ with $N=5$ as the function to optimize and train a 4 layer Multi-layer Perceptron with 96 neurons as the surrogate model. While Gradient Descent represents the steepest descent, Mind Mappings is able to use approximate gradients to perform well, especially compared to the unguided black-box approaches like Simulated Annealing.
%   }
%   \label{fig:motivation}
% \end{centering}
% \end{figure}

% For a given problem, $id_{target}$ and a target cost $c_{target}$, the search needs to find a mapping $m_{opt}$ that minimizes the distance between $f(m_{opt})$ and $c_{target}$.
% This step is based on the key insight that \emph{beyond simply being used to estimate cost $c$ for a given mapping $m$, the surrogate can also be used to estimate the change needed in $m$ such that it results in a target cost $c_{target}$.}

%In more detail,
\textbf{Gradient Descent with MLP-based Differentiable Surrogates.}
Section~\ref{subsec:func_approx} described the procedure to obtain a differentiable surrogate \fapprox \ by training an MLP to approximate the cost function.
We now use the surrogate to generate gradients that indicate the direction of steepest descent with respect to a \emph{candidate mapping} $m$, i.e.,  $\nabla $\fapprox$_{p_{id}}(m) = [\partial $\fapprox$/\partial m_0, .. , \partial $\fapprox$/\partial m_{D-1}]$. 
% based on the loss $\mathcal{L}$ 
$\nabla $\fapprox$_{p_{id}}$ is computed using the chain rule across layers of the MLP (surrogate), assuming the MLP parameters and $p_{id}$ are fixed.
%Conceptually, this is similar to applying back-propagation~\cite{backprop} algorithm with the MLP parameters and the $p_{id}$ fixed, while the input mapping vector $m_t$ made trainable, as depicted in Figure~\ref{fig:training}.

We use the generated gradients to perform a standard Gradient Descent starting from a randomly-chosen initial mapping $m@0$ (``$m$ at iteration 0''), setting $p_{id}=p_{target}$.
That is, we iteratively compute $\nabla $\fapprox$_{p_{target}}(m@t)$ and combine it with $m@t$ to form the next candidate mapping $m@{t+1}$.
This process is shown in more detail in Figure~\ref{fig:training}.

%Intuitively, during Phase 1, the surrogate model has been trained to learn the relation between each $m_i$ to the cost $f(m)$, which in Phase 2 is leveraged to estimate the change needed in each $m_i$ to drive $f(m)$ towards 
% the target cost $c\_{target}$.
%the minimum.
%This forms the core of our approach to realize a guided search.

\textbf{Projected Gradient Descent.} 
Applying Gradient Descent 
%\chris{is Gradient Descent capitalized or not?  inconsistent}\kartik{Done}
to mapping space search presents two issues.
First, after applying gradients, each value $m_d$ in the mapping 
vector falls potentially outside the domain of programmable attribute $P_d$.
%becomes a floating point value.
To address this, we round each $m_d$ to the nearest value in $P_d$.
%We round the floating point value to the nearest real value, based on the domain of the programmable attribute $P_d$.
%\chris{huh?  FP is a subset of the reals ... If what you meant by "real" was "valid value in the domain of said programmable attribute" LMK as I will need to go back and check 4.1.2.}\kartik{Yes, need to project back to a "real" that is in the $P_d$} \chris{I still don't understand}
Second, after rounding each $m_d$, the overall $m$ may be invalid with respect to $p_{target}$, i.e., $m \centernot\in M_{a,p_{target}}$.
To ensure the final mapping is valid, we check mapping validity of $m@t$ at each step $t$.
If validity fails, we calculate nearest neighbor valid mappings based on euclidean distance to $m@t$ and switch $m@t$ to the nearest valid mapping before continuing the search.
This is a standard approach, often referred to as \emph{Projected Gradient Descent}~\cite{projected_gradient_descent}, used in applications where gradient may steer the parameters out of the valid region~\cite{projected_0, projected_1}.
% and use nearest neighbor search.
% to project an invalid mapping to the closest valid one.
% That is, to check validity we de-normalize the attribute values in $m_t$ (invert the transformation from Section~\ref{sec:method:input_rep}) and call $\mathsf{isMember}$ as described in Section~\ref{sec:method:gen_train}.

\textbf{Avoiding Local Minimas.}
\label{subsec:local_minima}
Gradient Descent is infamous for getting stuck in local minima for non-convex optimization problems~\cite{local_minima} and our scheme runs the same risk.
To handle non-convexity, we introduce randomness at regular intervals throughout the search.
Specifically, we add an outer loop to the Gradient Descent algorithm described above, where after every $N$ iterations, a new random mapping vector is introduced.
The decision to replace the current mapping $m@t$ with the newly sampled valid mapping is based on a probability function $\mathsf{accept}$
%\chris{what does this function take as input?  It sounds like $t$.}\kartik{Some sort of temperature, prior value, current value. Do we want to elaborate?}
that helps us balance the trade-off between exploration and exploitation.
The choice of $N$ and the probability function is up to the implementation.
For example, the designer may choose to gradually
decay the probability of accepting a mapping with higher cost than the already-seen mappings over time, similar to Simulated Annealing.
We follow this strategy in Section~\ref{sec:eval}.

%\chris{this text looks stale.  please do a pass and while you are at it, update to the $m@t$ notation.}\kartik{Done}
Overall, Phase 2 performs the following steps until termination, given a target problem $p_{target}$:
\begin{enumerate}
\item Choose a random valid mapping vector $m@t$ where $t=0$.
    \label{phase2:step1}
\item Compute $c^*=$\fapprox$(m@t, p_{target})$ by forward propagation through the MLP.
%  Estimate the loss, $\mathcal{L}$ $(c*,c_{target})$.
\label{phase2:step2}
\item Derive gradients using back-propagation via the surrogate with respect to $m@t$, $\nabla = \partial $\fapprox$/\partial m@t$.
\item Update the mapping vector as $m@{t+1} = m@t - \alpha \nabla$, where $\alpha$ is a user-specified learning
rate.
\item Project $m@{t+1}$ to the valid target map space.
\item If $t\%N==0$, sample a random valid mapping $m_{rand}$. If $\mathsf{accept}(m_{rand}, m@t, T)$ returns true, update $m@{t+1}=m_{rand}$, where $T$ is a temperature term that is decayed over time.
\item Increment $t$ and go to Step~\ref{phase2:step2} until completion.
\end{enumerate}



==> problem.tex <==
\section{Problem Statement}
During the design process of a hardware accelerator, the architects typically have two decisions to make. 

\paragraph{Architecture} First, to choose architectural parameters to suit the budget and deployment requirements. These can include the number of processing elements, on-chip buffer sizes, network-on-chip type, bandwidth to off-chip memory to name a few. 
Let $A$ represent the architectural space of the exhaustive possibility of these hardware parameters at design time.

\paragraph{Schedule} As the next stage, for those chosen architectural parameters, the algorithm needs to be mapped --- which is the subject of this paper.
These scheduling parameters may be deduced: (1) in design time to be built into the hardware (2) in compile time to be mapped to the hardware, or (3) in run-time to dynamically to mapped to the hardware.
Let $S$ represent the schedule space of all the possible combinations of schedules.

Consider an architecture space $A$, where each architecture $a\in A$ has a schedule space $S$. Let a function $f$ estimate the cost vector $y$ for an input schedule $x\in S$, where the definition of \emph{cost} is upto the designer. Now, we can define the optimization problem that the designer needs to solve formally as Equation~\ref{eq:minmize}.
\begin{equation}
\displaystyle{\minimize_{a\in A} \ \minimize_{x\in S} \ f(a,x)}
\label{eq:minmize}
\end{equation}

The outer minimization problem includes several decisions that are tied to business, which is outside the purview of mathematics. Hence, we restrict our optimization search to finding the best schedule $x_{min}$ that achieves the target objective $y$ for a given architecture $a$, as depicted in Equation~\ref{eq:schedule}.

\subsection{Why is this a hard problem? }
The algorithm mapping to a specialized hardware has been a subject of extensive work in the recent time. Often referred to as the `dataflow', it dictates as to how the data is accessed, managed on-chip, delivered to the compute units, and how the compute is performed and written back.
Every variable that 
This mapping problem is a combinatorial optimization that is np-complete~\cite{npcomplete}, i.e., the solution can be verified in polynomial time. 
\begin{equation}
x_{min} = \argmin_{x\in S} f(a, x)
\label{eq:schedule}
\end{equation}


However, approaches to choose the mapping has either been based on expert designer choices or based on exhaustive searches. While exhaustive search is simply infeasible when all the parameters are enumerated, the designer choice may not be very optimal.
